Flexible sensitivity analysis for observational studies without observable implications

A fundamental challenge in observational causal inference is that assumptions about unconfoundedness are not testable from data. Assessing sensitivity to such assumptions is therefore important in practice. Unfortunately, some existing sensitivity analysis approaches inadvertently impose restrictions that are at odds with modern causal inference methods, which emphasize flexible models for observed data. To address this issue, we propose a framework that allows (1) flexible models for the observed data and (2) clean separation of the identified and unidentified parts of the sensitivity model. Our framework extends an approach from the missing data literature, known as Tukey's factorization, to the causal inference setting. Under this factorization, we can represent the distributions of unobserved potential outcomes in terms of unidentified selection functions that posit an unidentified relationship between the treatment assignment indicator and the observed potential outcomes. The sensitivity parameters in this framework are easily interpreted, and we provide heuristics for calibrating these parameters against observable quantities. We demonstrate the flexibility of this approach in two examples, where we estimate both average treatment effects and quantile treatment effects using Bayesian nonparametric models for the observed data.

==> sections/app-latent-confounder-examples.tex <==
\section{Additional Latent Confounder Examples}

\textbf{Example: Binary Potential Outcome, Binary Latent Confounder, No Covariates:}
% Main points:
% \begin{itemize}
% \item Introduce R\&R model.
% \item Show that with no covariates, there is no identification with binary outcomes because the parameters of a mixture of a Bernoulli are not identified.
% \item Tease the fact that when there are parameters and a parametric model for $U$ that is constant across covariates that you will end up with identification.
% Move the full argument and plot to appendix.
% \end{itemize}
% \avi{placeholder} We discuss the implications of the latent confounder formulation for a binary outcome. In this case, the outcome distribution is still Bernoulli since a mixture of Bernoullis is still Bernoulli.
%\textbf{Binary latent confounder and binary potential outcomes:} 
One of the best-known instances of likelihood-based sensitivity analysis is the latent confounder model introduced in \citet{rosenbaum1983assessing}, which generalized the sensitivity analysis of \citet{cornfield1951}.  This model considered the case where the outcome, treatment, and latent variable are all binary.
We will show that this sensitivity model does not suffer from partial identification issues when there are no covariates.
%
\begin{align}
U &\sim f(U)\label{eqn:binary1}\\
T \mid U &\sim Bern(g(\alpha + \psi_T U))\label{eqn:binary2}\\
Y(t) \mid U &\sim Bern(g(\beta_{t} + \psi_{Yt} U))\label{eqn:binary3}
\end{align}

Where $g$ is a smooth, monotonically increasing link function.
Rosenbaum and Rubin stratified the population by the propensity score $e(X)$ and proposed this model with binary $U$. 
Without loss of generality, they set the link functions $g$ to be the inverse-logit function.  Here, there are three sensitivity parameters $\psi_T$ and $\psi_{Yt}$ describing the relationship of the unobserved confounder to the treatment assignment and potential outcomes.
When either $\psi_T$ or the pair of parameters $\psi_{Yt}$ are set to 0, this model describes an unconfounded observational study.
In such cases, the model could be fully specified just in terms of $\alpha$ and $\beta_t$.
For this reason, we call $\alpha$ and $\beta_t$ the \emph{unconfounded parameters}.

The sensitivity parameters in this model are unidentified in the presence of the unconfounded parameters. 
We state this formally as follows.

\begin{proposition}
Under the model specified by \eqref{eqn:binary1}--\eqref{eqn:binary3},
for any  observed data distribution $f(Y^{obs}, T)$, for any arbitraty setting of the sensitivity parameters $\pi_u$, $\psi_T$, and $\psi_{Yt}$, there exists a setting of the unconfounded parameters $\alpha$ and $\beta_t$ that generates the observed data distribution.
\begin{proof}
We give a sketch of the proof here and the full proof in the appendix.
Under this model, after integrating out $U$, the treatment $T$ and observed outcomes $Y^{obs}$ are both mixtures of Bernoullis, which are themselves Bernoullis.
Thus, the three probabilities $P(T = t)$ and $P(Y(t) = 1 \mid T = t)$ for $t \in \{0, 1\}$ fully characterize the observed data distribution.
We will call these the ``observed-data probabilities.''
It can shown that, for any setting of the sensitivity parameters, the unconfounded parameters can be set to induce aribitratry observed-data probabilities.
%Thus, the observed-data probabilities do not identify the sensitivity parameters in the presence of the unconfounded parameters. 
\end{proof}
\end{proposition}

Thus, the observed data carry no information about the sensitivity parameters, even as the sample size grows to infinity.

We show this through a decomposition into \eqref{eqn:obs_distribution} and \eqref{eqn:obs_distribution}
The marginal probability of treatment is

\begin{align}
\label{eqn:pi_t}
T &\sim \text{Bern}(\pi_t) \nonumber\\
\pi_t &= \pi_u g(\alpha + \psi_T) + (1-\pi_u)g(\alpha) 
\end{align}

This implies the following conditional distribution of the latent confounder using \eqref{eqn:confounder_conditional}:

\begin{align}
\label{eqn:latent_bernoulli_posterior}
U\mid T &\sim \text{Bern}(h(T, \pi_u, \psi_T, \alpha)) \nonumber\\
h(T, \pi_u, \psi_T, \alpha) &= \frac{\pi_u(g(\alpha + \psi_T)^T + (1-g(\alpha + \psi_T))^{1-T})}{\pi_t^T(1-\pi_t)^{1-T}}.
\end{align}

 By \eqref{eqn:obs_distribution} we can write the observed data distribution as a mixture of Bernoulli random variables, which is itself Bernoulli:

\begin{align}
Y(t) \mid T=t &\sim h(T, \pi_u, \psi_T, \alpha)\text{Bern}(g(\beta_t +  \psi_Y)) + (1-h(T, \pi_u, \psi_T, \alpha))\text{Bern}(g(\psi_Y)) \nonumber\\
&\sim \text{Bern}\left(h(T, \pi_u, \psi_T, \alpha)g(\beta_t +  \psi_Y) + (1-h(T, \pi_u, \psi_T, \alpha))g(\beta_t)\right) \label{eqn:y_obs_rr} \nonumber\\
&\sim \text{Bern}(\pi_{Y(t)_{\text{obs}}})).
\end{align}

Putting these together, the observed data density $f(Y^{obs}, T)$ is fully characterized by a $2 \times 2$ table of probabilities, satisfying:
\begin{align}
p_{t, y^{obs}} = \pi_t^{t}(1-\pi_t)^{1-t} \cdot \pi_{Y(t)_{\text{obs}}}^{y^{obs}}(1-\pi_{Y(t)_{\text{obs}}})^{1-y^{obs}}.
\label{eqn:RR relation}
\end{align}
This table has 3 degrees of freedom.
Thus, the 3 unconfounded parameters $\alpha$, $\beta_0$, and $\beta_1$ are sufficient to satisfy \eqref{eqn:RR relation} when the 4 sensitivity parameters $\pi_u$, $\psi_T$, $\psi_{Y0}$ and $\psi{Y1}$ are fixed at arbitrary values.



For any table of probabilities $(p_{00}, p_{01}, p_{10}, p_{11})$, and for any setting of the sensitivity parameters $\pi_u$, $\psi_T$, $\psi_{Y0}$, and $\psi_{Y1}$, there exists a set of parameters $\alpha$, $\beta_0$, $\beta_1$ 

%The observed data distribution for treatment $t$ can be represented as two-component mixture of Bernoulli random variables.  %The second line follows because a mixture of Bernoulli random variables is itself Bernoulli.  %Although the functional dependence of the observed data on the relevant parameters is complicated, it is important to note that the observed data outcome probability, $P(Y(t)=1 \mid T=t) = h(T, \pi_u, \alpha, \psi_)g^{-1}(\beta_t +  \delta_t) + (1-h(T, \pi_u, \alpha, \psi_))g^{-1}(\beta_t)$, is identifiable.  

Finally, since 
$$\pi_{Y(t)_{\text{obs}}} = h(T, \pi_u, \psi_T, \alpha)g(\beta_t +  \psi_Y) + (1-h(T, \pi_u, \psi_T, \alpha))g(\beta_t)$$


As shown in \citet{rosenbaum2002covariance}, for fixed values of the sensitivity parameters, $\alpha$, and $\beta_t$ are identified.
This is evident because the observed data identifies the marginal treatment assignment probability $\pi_t$ and the observed data outcome probabilities $\pi_{Y(t)_{\text{obs}}}$.
More importantly, the maximum likelihood for $\alpha$ and $\beta_t$ takes on the same value for any settings of the sensitivity parameters because Equation \ref{eqn:pi_t} is a continuous monotone increasing function in $\alpha$ with range $(0, 1)$ for any fixed values of $\alpha$ and $\pi_u$.  Similarly, Equation \ref{eqn:y_obs_rr} is a continuous monotone function of $\beta_t$ for $h$ and $\psi_Y$ fixed.  This means that the sensitivity parameters are completely unidentified. 

\textbf{Binary Outcome, Normal Confounder, No Covariates:}
We follow the same model as above but instead of a binary latent confounder we posit the existence of a normally distributed latent confounder, $U \sim N(0,1)$ and let $g(x) = \Phi(x)$ be the probit function (rather than the inverse-logit). Then,

\begin{align}
\pi_t &= \Phi \left( \frac{\psi_T}{ \sqrt{1+\psi_T^2} } \right)\\
f(U \mid T=1) &\propto \phi(U)\Phi(\psi_T + \psi_T U)\\
\pi_{Y(t)_{\text{obs}}} &= E[g(\beta_t + \psi_Y U) \mid T = t]
\end{align}

\noindent where $f_u(U \mid T)$ is known as the extended skew normal distribution \citep{azzalini2005skew}.  Again, $\pi_t$ is a continuous monotonic function of $\psi_T$ for any fixed $\alpha$.  $\alpha$ is not identified from the observed data, but for $\alpha$ fixed to any value, $\psi_T$ is identified.  Similarly we can use equation \ref{eqn:obs_distribution} to argue that $\pi_{Y(t)_{\text{obs}}}$ is monotonic in $\beta_t$, $\psi_Y$ is completely unidentified and that $\beta_t$ is identified given $\psi_Y$.   
%\avi{I really like this example, but don't totally follow the argument. It's still a mixture of Bernoullis -- and hence Bernoulli -- but the sensitivity parameters are still identified. We need to take a stand on how much this matters.}

%\begin{theorem}
%Assume without loss of generality, there exists a univariate random variable $U$ for which $Y(0)_i, Y(1)_i %\independent T \mid U, X$. Further assume that $Y(t) \mid X, g(\xi^yU) $ and that $P(T \mid U, X) \neq P(T \mid %X)$.  Then the observed data distribution, $Y(t) \mid X, T=t$ depends on $\xi^Y$.  Further $\xi^Y$ is identifiable.
%\end{theorem}

% As we will see in the next example, it is not generally the case that the sensitivity parameters in a latent confounder formulation are unidentified. The unidentifiability in the Bernoulli outcome model results directly from the fact that a mixture of Bernoulli random variables is itself a Bernoulli random variable.  Similarly motivated latent confounder models for non-binary potential outcomes often imply sensitivity parameters which are at least partly informed by the data.  


==> sections/latent-class-model.tex <==
\section{A Latent Class Model}
\label{sec:mix-model}
%\damour{I think we uniformly agree that this section should be cut or appendixed.}

In this section, we propose an alternative family of tractable extrapolation models motivated by binary latent confounder models (e.g. Example 1, Section \ref{sec:latent-confounder}).  Unlike previous latent confounder approaches, our approach does not induce partial identification of the sensitivity parameters.  An interesting consequence of the latent class models we propose is that, in contrast to the logistic-EF models, the selection functions asymptote at values \emph{strictly} between 0 and 1.  As a result the models induce bounded ignorance regions for the causal estimands even when the sensitivity parameter range is unbounded. 

\subsection{Model specification}
 Binary latent confounder models imply that the observed and missing data distributions are two component mixtures with the same component distributions but different mixture weights.  This forms the starting point for the proposed model:
%
%Specifically, we demonstrated that a binary latent confounder implies a two component mixture model, e.g. a mixture of Bernoulli random variables \citep{rosenbaum1983assessing} or a two component mixture of normal distributions \citep{imbens2003sensitivity, dorie2016flexible}. For example, in the normal potential outcome model (Equation \ref{eqn:dorie_model}) the means and variances of the normal components are identical for both the observed and missing potential outcomes distributions but the mixture weights differ. 
%
%
\begin{align}
\label{eqn:mixture}
f^{\rm obs}(Y(t) \mid T=t, X) = \pi_{tX}^1 f_0(Y(t)) + (1-\pi_{tX}^1)f_1(Y(t)) \\
f^{\rm mis}(Y(t) \mid T=1\-t, X) = \pi_{tX}^0 f_0(Y(t)) + (1-\pi_{tX}^0)f_1(Y(t))
\end{align}
%
\noindent where $\pi_{tX}^t$ and $\pi_{tX}^{1\-t}$ correspond to the mixture weights for the observed and missing data distributions in treatment arm $t$.  The mixtures weights are allowed to depend on $X$. $\pi_{tX}^{1\-t}$ is unidentifiable, whereas  $\pi_{tX}^t$ is identifiable given certain assumptions about the mixtures densities $f_0$ and $f_1$.  By convention we assume the median of $f_0(Y(t))$ is less than the median of $f_1(Y(t))$ and define $U(t) \in \{0, 1\}$ to be a latent class indicator corresponding to the two mixture components with $f(Y(t) \mid U(t) = u, T=t, X) =:  f_u(Y(t) \mid X, T=t)$.  Given $U(t)$ and $X$, unconfoundedness is satisfied: $f(Y(t) \mid U(t), X, T) = f(Y(t) \mid U(t), X)$.  Then, the treatment assignment function implied by Equation \ref{eqn:mixture} is
%
\begin{align}
\label{eqn:mix-selection}
&f(T = 1 \mid Y(t), X) =\\ 
&\frac{p_1\left[\pi_{tX}^1f_0(Y(t)) + (1-\pi_{tX}^1)f_1(Y(t))\right]}{p_1\left[\pi_{tX}^1f_0(Y(t)) + (1-\pi_{tX}^1)f_1(Y(t))\right] + (1-p_1)\left[\pi_{tX}^{0}f_0(Y(t)) + (1-\pi_{tX}^{0})f_1(Y(t))\right]} \nonumber
\end{align}
%
\noindent with $p_1 = f(T=1)$.  The following theorem describes the behavior of this treatment assignment function.
\begin{theorem}
\label{thm:mix_sel}
If $\lim\limits_{Y(t) \to -\infty} \frac{f_1(Y(t))}{f_0(Y(t))} \to 0$ and $\lim\limits_{Y(t) \to \infty} \frac{f_0(Y(t))}{f_1(Y(t))} \to 0$, then $\lim\limits_{Y(t) \to -\infty} f(T=1\mid Y(t)) \to (0 < k_{-\infty} < 1)$ and $\lim\limits_{Y(t) \to \infty} f(T=t\mid Y(t)) \to (0 < k_\infty < 1)$ with $k_{-\infty} = \frac{p_1 \pi_{tX}^1}{p_1 \pi_{tX}^1 + (1-p_1)\pi_{tX}^0}$ and $k_\infty = \frac{p_1 (1-\pi_{tX}^1)}{p_1 (1-\pi_{tX}^1) + (1-p_1)(1-\pi_{tX}^0)}$.  $k_{-\infty} < k_\infty$ if and only if $\pi_{tX}^0 \geq \pi_{tX}^1$ with equality when $\pi_{tX}^1=\pi_{tX}^0$ corresponding to unconfoundedness.
\end{theorem}

Unlike the logistic treatment assignment models, this assignment mechanism asymptotes at values strictly greater than 0 and strictly less than 1.  The behavior of these assignment mechanisms can be further understood in terms of the following lemma:

\begin{corollary}
Under the conditions stated in Theorem \ref{thm:mix_sel}, we have
\begin{align}
&\frac{f(T=1 \mid Y(t) = +\infty, X)}{f(T=0 \mid Y(t) = +\infty, X)} \Bigg/  \frac{f(T=1 \mid Y(t) = -\infty, X)}{f(T=0 \mid Y(t) = -\infty, X)} \nonumber\\
&= \frac{ \mathrm{odds}(U(t) = 1 \mid X, T=t) }{ \mathrm{odds}(U(t) = 1 \mid X, T=1\-t) } \nonumber\\
&= \frac{\pi_{tX}^1}{\pi_{tX}^0}\Bigg/\frac{1-\pi_{tX}^0}{1-\pi_{tX}^1}
\end{align}
\label{cor:mix_odds_ratio}
\end{corollary}
%
\noindent The odds ratio of treatment for very large $Y(t)$ versus very small $Y(t)$ is a finite constant.  By contrast, in the logistic model specified in Equation \ref{eq:exp-log-sel} the odds diverge to either 0 or $\infty$ as $Y(t) \to \pm \infty$.  

\subsection{Parameter interpretation and calibration}  
\label{sim:calibration}
We propose an interpretable sensitivity specification for the mixture weights: %
\begin{align}
\label{eqn:mix_sel_fn}
f(U(t) = 0 \mid X, T) &= \text{logit}^{-1}(\alpha_t(X) + \omega_t I\{T=1\-t\})
\end{align}
\noindent $\alpha_t(X)$ is the regression surface for the observed covariates and $\omega_t$ corresponds to the log odds ratio of the mixture weights from the observed and missing data components (in this case independent of $X$).  By specifying $\omega_t$, we posit that the odds ratio of the class probabilities for the observed and missing data distributions is
\begin{equation}
\label{eqn:omega_t}
\exp(\omega_t) = \frac{\pi_{tX}^1}{\pi_{tX}^0}\Bigg/\frac{1-\pi_{tX}^0}{1-\pi_{tX}^1} 
\end{equation}

Under the conditions stated in Theorem $\ref{thm:mix_sel}$ and by Corollary \ref{cor:mix_odds_ratio}, $\omega_t$ corresponds to the log-odds ratio of an $X$-matched pair being assigned treatment, given divergent potential outcomes.  The proposed latent class model resembles Rosenbaum's $\Gamma$, in which the investigator proposes a bound, on the chances of matched units receiving treatment \citep{rosenbaum2002covariance, keele2010overview}.  Note that under this model, average and quantile treatment effects are bounded because $\omega_t \to \infty \implies U(t) \to 0$ and $\omega_t \to -\infty \implies U(t) \to 0$. The quantiles of $Y(t)$ are maximized when $f(U(t) = 1 \mid T=1\-t) = 1$ and minimized when $f(U(t) = 0\mid T=1-t) = 1$, i.e. the missing data belong to a single latent class with probability one. In other words, unlike the logit-EF models, the mixture selection model implies a bounded ignorance region for treatment effects.  The implications of these observations fact are explored in detail in the simulated data analysis in Section \ref{sec:analysis_simulation}.  
% In the Section below, we describe how to calibrate sensitivity parameters in both the logistic-EF models and the latent class models. 

\hfill \break
\noindent \textbf{Calibration in the Latent Class Specification:} As with calibration for the logistic-EF models, we calibrate the sensitivity parameters against estimable coefficients for the standardized observed covariates, $ X$.  In this model, rather than regressing $ X$ on the observed treatment assignment, $T$, we consider the regression of $X$ on the latent class indicator $U(t)$.  First, we estimate the observed data conditional distributions $f(Y(t) \mid  X, T=t)$ as a two component mixture with mixture weights which are logistic in $ X$.  
%\begin{equation}
%\label{eqn:tilde_gamma_mix}
%\omega_t = \log \left(\frac{ \mathrm{odds}(U(t) = 1 \mid \hat \alpha + \hat \beta X, T = t) }
%{\mathrm{odds}(U(t) = 1 \mid \hat \alpha  + \hat \beta X, T = (1\- t)}\right) 
%\end{equation}
%Again, $ Y(t)$ is the rescaled potential outcome, and $\gamma_t$ is chosen according to the solution the equation ${\gamma}_t = \gamma_t\sigma_{yt}(\gamma_t)$.  
Then we propose values for the unidentified mixture weights for the missing data density  $\omega_t$ where
%
\begin{align}
\label{eqn:mix_sel_fn}
\pi_{tX}^0 = f(U(t) = 0 \mid  X, t) &= \text{logit}^{-1}(\alpha_t(X)  X + \omega_t I\{T=1\-t\})
\end{align}
\noindent where $\omega_t$ has the interpretation given in Equation \ref{eqn:mix-selection}. The missing data mixture weights depend on both the standardized covariates, $ X$, and the indicator for the treatment assignment.  Specifying $\omega_t$ completes the specification of the treatment assignment function (Equation \ref{eqn:mix_sel_fn}).  %We summarize the calibration method in Algorithm \ref{algo:mix-calibration}.  

% \begin{algorithm}

% \caption{Sensitivity Parameter Calibration in the Mixture Model}
%   \begin{enumerate}
%     \item Fit a mixture model to the observed data with mixture weights that are logistic in $\tilde X$
%     \item Calibrate $\omega_t$ relative to the coefficients $\hat{\beta}$
%     \item Compute $f(Y(t) \mid T = (1 - t),  \omega_t, X)$, estimate treatment effects.
% \end{enumerate}
% \label{algo:mix-calibration}
% \end{algorithm}


\subsection{Simulated Data Analysis}
\label{sec:analysis_simulation}


\begin{figure}[h!]	
	\begin{subfigure}[t]{2.8in}
		\centering
		\includegraphics[width=2.4in]{figs/mix_missing_plot.pdf}
		\caption{$P(T=0 \mid Y(0), X=0)$, mixture selection}\label{fig:treat_prob_mix}
	\end{subfigure}
    \quad
		\begin{subfigure}[t]{2.8in}
		\centering
		\includegraphics[width=2.4in]{figs/simulation_ribbons.pdf}
		\caption{Quantile effects, mixture selection}\label{fig:sim_ribbons}		
	\end{subfigure}	\\
	
	\vspace{.2in}
	
	\begin{subfigure}[t]{2.8in}
		\centering
		\includegraphics[width=2.4in]{figs/mix_missing_plot_logit.pdf}
		\caption{$P(T=0 \mid Y(0), X=0)$, logistic selection}\label{fig:treat_prob_logit}
	\end{subfigure}
    \quad
		\begin{subfigure}[t]{2.8in}
		\centering
		\includegraphics[width=2.4in]{figs/simulation_ribbons_logit.pdf}
		\caption{Quantile effects, logistic selection}\label{fig:sim_ribbons_logit}		
	\end{subfigure}	\\
	
	\caption{Example selection functions and missing potential outcome densities for control potential outcomes (a, c) and 95\% posterior confidence bands for $\tau_q$ (b, d) for two model specifications.    a) The latent class selection mechanism implied by Equations \ref{eqn:mix-selection} and \ref{sim:model_spec} and implied missing control potential outcome densities at $X=0$.  Treatment assignment probabilities asymptote at values strictly greater than 0 and less than 1 for all values of $Y(0)$. b)  95\% posterior confidence bands for $\tau_q$ in the latent class model. When unconfoundedness holds, $\omega_0, \omega_1 = 0$ and the inferred treatment effects are significantly negative at all quantiles.  Dashed lines represent quantile treatment effects when $(\omega_0, \omega_1) = (\pm \infty, \mp \infty)$ in the treatment assignment model \ref{eqn:mix_sel_fn}. c) Logistic selection mechanism and implied missing control potential outcomes at $X=0$.  Treatment assignment probabilities diverge to 0 and 1. d)  95\% posterior confidence bands for $\tau_q$ under logistic selection for the same observed data model. The magnitude of the quantile effects grow monotonically in the absolute difference between $\gamma_1$ and $\gamma_0$.  Unlike with the latent class model the effects are unbounded in the logistic model. \label{fig:simulation}}
\end{figure}





%In the previous example we explored an application of the extrapolization factorization for non-parametric modeling of the mean response surface, but assumed a normally distributed residual potential outcome distribution.  
We now provide a simple example demonstrating sensitivity analysis with the latent class model and compare the approach to the logistic specification introduced previously.  In this simulation, we generate data from a latent class model with a single observed covariate:
% 
\begin{align}
\label{sim:model_spec}
    f(T) &\sim \text{Bern(1/2)}\nonumber\\
    f(X \mid T) &\sim 
\begin{cases}
N(-1, 1)\quad &T=1\\
N(1, 1)\quad &T=0\\
\end{cases} \nonumber\\
    f(U(t) \mid X, T) &\sim 
\begin{cases}
\text{Bern}(\text{expit}(\beta X + \omega_1 I\{ T = 1\} + \tau))\quad &t=1\\
\text{Bern}(\text{expit}(\beta X + \omega_0 I\{T=1\}))\quad &t=0\\
\end{cases} \nonumber\\
f(Y(t) \mid U(t)) &\sim
\begin{cases}
N(\mu_{1t}, \sigma_{1t})\quad U(t)=0\\
N(\mu_{2t}, \sigma_{2t})\quad U(t)=1
\end{cases} 
\end{align}
%
where  $U(t)$ is a latent class in treatment arm $t$ and $\tau$ correspond to a treatment effect on the latent class probability.  The distribution of the latent class variable is potentially different in the treatment and control arms even after controlling for observed covariates.  However, in this simulation we assume the the latent class distributions are the same for both potential outcomes.\footnote{This assumption is testable from the observed data.}  We then simulate 1000 observations using the following data generating parameters: $(\mu_1, \sigma_1) = (0, 1)$, $(\mu_2, \sigma_2) = (5, 2)$, $(\omega_0, \omega_1) = (1, 1)$ and $\beta = 1$, $\tau = 0$.  For this data generating procedure, $\tau=0$ means zero quantile treatment effect: $\tau_q =  0$ for all $q$ because $f(U(0) \mid X, T) = f(U(1) \mid X, T)$.  

In this section, we illustrate how to conduct a sensitivity analysis in such a model and contrast the approach to the logistic-EF model proposed in Section \ref{sec:logit-ef}.  First, we estimate the observed data densities $f^{\rm obs}(Y(t) \mid X, T=t)$ for the binary latent class model using the probabilistic programming language STAN \citep{stan}.  %We plot inferred observed data densities at different levels of $X$ for both potential outcomes in Figure \ref{fig:YvXsim}.  
Consistent with the true data generating process, we use the selection model specified in Equation \ref{eqn:mix_sel_fn}.  In this model the sensitivity parameters are:
%
\begin{align*}
\omega_0 &= \log\left(\frac{p(U(0) = 1 \mid T=0, X=x)}{1-p(U(0) = 0) \mid T=0, X=x)} \Bigg/\frac{p(U(0) = 1 \mid T=1, X=x)}{1-p(U(0) = 1 \mid T=1, X=x)}\right) = 1\\
\omega_1 &= \log\left(\frac{p(U(1) = 1 \mid T=1, X=x)}{1-p(U(1) = 0 \mid T=1, X=x)} \Bigg/ \frac{p(U(1) = 1 \mid T=0, X=x)}{1-p(U(1) = 1 \mid T=0, X=x)}\right)  = -1 \hspace{.15in} \forall x
\end{align*}
%
The log odds ratios for the latent class, $\omega_t$, are unidentifiable from the observed data.  In practice, we can calibrate $\omega_t$ using the the coefficient of determination, as described in Section \ref{sec:calibration}.  %In this simulation study, we assume the additional change in log odds of $U(t)$ in the missing data component, conditional on $X$, on  will be no larger in magnitude than $\hat \beta$. 
To illustrate the full generality of our approach to sensitivity analysis, we evaluate quantile treatment effects for different values of $\omega$: for a given estimate of the complete data densities, we numerically estimate the quantile treatment effects for a range of quantiles.  

By way of illustration, in Figure \ref{fig:treat_prob_mix} we depict the selection function $f(T \mid Y(0), X=0)$ and implied missing control potential outcome densities, $f^{\rm mis}(Y(0) \mid T=1, X=0)$ for different levels of $\omega_0$.  In Figure \ref{fig:sim_ribbons} we plot the posterior distribution of the quantile treatment effects at for four different values of ($\omega_0, \omega_1$).  The upper and lower dashed lines in Figure \ref{fig:sim_ribbons} correspond to the upper and lower bounds on the quantile treatment effects, with the the upper line reflecting $\tau_q$ for $(\omega_0, \omega_1) = (\infty, -\infty)$ and the lower dashed line $\tau_q$ for $(\omega_0, \omega_1) = (-\infty, \infty)$.  Thus, the latent class model implies a bounded ignorance region for the quantile treatment effects.

For comparison, we also compute the posterior distribution of $\tau_q$ under the logistic selection function for the same observed data model.  As shown in the normal mixture example, Equation \ref{eqn:mix_normal_dists} of Section \ref{sec:logit-ef}, when the observed potential outcome is a mixture of exponential families, the missing potential outcomes are also a mixture of the same exponential family class.  In Figure \ref{fig:treat_prob_logit} we plot example logistic selection functions and implied missing control potential outcome densities. Unlike the selection function in the latent class model, the logistic selection function changes the mixture component means in addition to the mixture weights.  In fact, $\underset{\gamma_t \to \pm \infty}{\lim} E[Y(t) \mid T=1\-t, X] \to \pm \infty$.  Thus, as $|\gamma_0 - \gamma_1|$ grows, the magnitude of the quantile treatment effects increase without bound.  Figure \ref{fig:sim_ribbons_logit} depicts the posterior distribution of quantile treatment effects for different values of $(\gamma_0, \gamma_1)$.  As shown, the quantile treatment effect can exceed the bounds implied by the most extreme sensitivity parameters in the latent class model.  

The ease with which we can evaluate sensitivity for different selection specifications highlights an additional strength of our approach.   By separating observed data modeling from the sensitivity analysis, we can easily evaluate the sensitivity of our results under a range of assumptions about the selection function without re-fitting potential outcome models.  Generating all of the results presented in this section meant running MCMC sampling exactly once to estimate the observed data densities.  This stands in contrast to the latent confounder models described in Section \ref{sec:latent-confounder}, in which the models must be re-fit for each new setting of the sensitivity parameters.


%\begin{figure}	
%	\centering
%	\includegraphics[width=5.5in]{figs/simulation_ribbons.pdf}
%	\caption{(a) Treatment assignment probabilities, $P(T \mid Y(t), X)$, for $\omega_t \in \{-1, 0, 1\}$.  (b) 95\% posterior bands for estimated %quantile treatment effects for different values of the odds ratio sensitivity parameters.  At the true values, $(\omega_0, \omega_1) = (-1, 1)$, we %recover 0 quantile treatment.  Under unconfoundedness, $(\omega_0, \omega_1) = (0, 0)$, the posterior mean quantile treatment effect is significantly negative.}
%	\label{quant_sens}
%\end{figure}


%Exponentially modified Gaussian distribution
%\begin{align*}
%    f(T) &\sim \text{Bern(logit}^{-1}(f(X))) \\
%    f(T \mid Z) &\sim \text{Bern(logit}^{-1}(f(Z))) \\
%    f(Y(t) \mid Z, T=t) &\propto ZN(\mu_1, \sigma_1) + (1-Z)N(\mu_2, \sigma_2)
%\end{align*}


% \subsection{Independent potential outcomes}

% First, assume the potential outcomes are uncorrelated conditional on treatment assignment. This would arise for instance, if there was a binary latent variable that was perfectly correlated with treatment assignment (see latent variable formulations).  

% Then, by Equation \ref{eqn:selection_decomposition_ind}

% $$ f(T \mid [Y(0), Y(1)]) \propto \frac{exp(\alpha^{*} + \beta_0 X + \beta_1 X + \gamma_0 Y(0) + \gamma_1 Y(1))}{1 + exp(\alpha^{*} + \beta_0 X + \beta_1 X +  \gamma_0 Y(0) + \gamma_1 Y(1))}$$



% Which corresponds to a simple location shift of the mean of each normal.  

% \begin{align}
% f(Y(1) - Y(0) \mid T=1, X) &= f_{\text{normal}}(\mu_1(X) - \mu_0(X) - \sigma_1^2\gamma_0, \sigma_1^2)\\
% f(Y(1) - Y(0) \mid T=0, X) &= f_{\text{normal}}(\mu_1(X) + \sigma_0^2\gamma_1 - \mu_0(X), \sigma_0^2)
% \end{align}

% We demonstrate this for different choices of $\gamma$ in the blood pressure example from \citep{dorie2016flexible}.

% TODO














==> sections/latent-confounder-scratch.tex <==



\subsection{Scratch below}


The latent confounder formulation implies that, once the latent variable $U$ is integrated out, the distributions of potential outcomes are mixtures over the latent variable $U$.
\begin{align}
%f_{\psi_T}(T \mid X) &= \int_{\mathcal U}f_{\psi_T}(T \mid U, X) f(U \mid X)dU
%\label{eqn:obs_T_distribution}\\
f_\psi(Y(t) \mid X, T) &= \int_{\mathcal U} f_{\psi_{Yt}}(Y(t) \mid X, U)f_{\psi_T}(U \mid X, T) dU. \label{eqn:PO_distribution}
\end{align}
\noindent Later, we use this mixture representation to establish identification results using results from the mixture modeling literature.


We discuss two related difficulties that stem from the fact that the complete-data model is related to the observed data model by a non-trivial marginalization:
%$$
%\underbrace{f(Y^{obs}, T \mid X)}_{\text{Observed data density}}
%= \int \underbrace{f([Y^{obs}, Y^{mis}], T \mid X)}_{\text{Complete data density}}
%dY^{mis}.
%$$
$$
\underbrace{f(Y(T), T \mid X)}_{\text{Observed data density}}
= \int \underbrace{f([Y(T), Y(1-T)], T \mid X)}_{\text{Complete data density}}
dY(1-T).
$$

It is difficult to specify a flexible complete-data model when only the margin is testable.

It is difficult to specify a parametric complete-data model that satisfies the margin constraint.



%any complete data model can be factored into two pieces:
%%$$
%%f([Y(t), Y(t-1)], T \mid, X) = \underbrace{f(Y(T), T \mid X)}_{\text{Observed data}} \cdot
%%\underbrace{f(Y(1-T) \mid Y(T), T, X)}_{\text{Missing outcome}}.
%%$$
%%In the missing data literature, this factorization is referred to as the pattern-mixture factorization.
%The first factor is the density of the observed data, given by the treatment assignment $T$ and the observed potential outcome $Y(T) = Y^{obs}$.
%The second factor is the conditional density of the missing potential outcome $Y(1-T)$, given all observed data.

Without parametric assumptions, the missing outcome factor is completely unidentified by the data.
This has two major implications.
First, it implies that a complete-data model cannot be fully nonparametric, because the data cannot speak about the unidentified factor.
Thus, modern techniques for trading off bias and variance in model fitting can only be applied to the observed data portion of the model.
Secondly, 



\begin{itemize}
    \item Difficult to specify a complete-data model family under the constraint that the complete-data models integrate to the same observed-data model. 
    \item Difficult to specify a flexible complete-data model -- cannot use tools like cross-validation to trade off misspecification bias and variance.
    Can only do this for observed data model.
\end{itemize}
We then describe some of the difficulties involved in specifying sensitivity models with unidentified sensitivity parameters under current frameworks.
In particular, we show that in many cases, latent confounder specifications often induce substantively different observed data distributions depending on the values of the sensitivity parameters.
We demonstrate this problem with examples and theory.


Section outline:
\damour{This is to be implemented. Section headers are currently in place, but prose has not been replaced.}
\begin{itemize}
    \item Short description of what is wrong, in principle, with identified sensitivity parameters.
    \item Latent confounder models. Pared down section 2.2 + Deep demonstration of all sub-points with normal example without covariates (current section 2.4). Show that this yields a mixture. Clearly, one of the unobserved confounder models fits the mixture distribution better than the unconfounded version.
    \item Some more examples with covariates.
    \item When are sensitivity parameters identified? Current section 2.4.
\end{itemize}

%\avi{This section should be something like ``what's wrong with latent confounder models?'' and then break it down point by point. In the sketch of the intro, we have a few issues that we raise, but they don't really appear here: (1) Conflates posterior uncertainty with sensitivity/ignorance; (2) Observed data fit depends on sensitivity parameter setting; (3) Computationally inefficient: New estimation for each $\gamma$ setting}

%\avi{As written, this is really all about \#2, but we don't really emphasize the consequences part.}

%\avi{What about $\psi$-conditional and $\g-marginal?}
\subsection{Implications of Partial Identifiability}

What sorts of mistakes do we make when we mix up model selection and sensitivity analysis?
\begin{itemize}
\item Mixing up variation in causal effect estimates from observed data model specification (testable) and latent confounder specification (not testable).
\item These factors can push treatment effect variation in the same or opposite directions, resulting in over-stated or under-stated sensitivity to latent confounding.
\item Preventable vs unpreventable ignorance.
\item Can make statements like ``the data support unconfoundedness'', but this is using parametric assumptions to test a non-parametric assumption. Mixes types of assumptions when doing robustness checking. 
\item Sensitivity analysis is itself sensitive to misfit and parametric specification.
\end{itemize}


Partial identification is not simply a mathematical curiosity-- it has real implications for the way sensitivity analysis is conducted and interpreted.
For example, it is common to assess sensitivity by estimating causal effects for a range of sensitivity parameters, but when there is partial identification, the results can be misinterpreted.
As we have demonstrated in Figure \ref{fig:misfit}, the implied observed data density changes as a function of the sensitivity parameters, and thus some settings of the sensitivity parameters may be inconsistent with the true observed data density.
Here, there is a conflation between estimation uncertainty and model ignorance.
Moreover, partial identification has computational implications.
When the observed data likelihood is not invariant to changes in the sensitivity parameters the model must be re-fit for each setting of the sensitivity parameters.
Following \citet{linero2017bayesian} and \citet{gustafson2018sensitivity}, and motivated by these problems we argue that in general 1) the sensitivity parameters should be unidentified and 2) the treatment effects should be identified conditional on the sensitivity parameters.
Below, we introduce the extrapolation factorization for causal inference, which satisfies these criteria.  



\franks{I moved this from intro down here. May want to integrate it with 2.5.  "Concretely, we propose a distribution for the latent variable $U$, such that $T \text{ }\independent\text{ } [Y(0), Y(1)] \mid X, U$.  One of the most well known examples of latent confounder-based sensitivity analysis, \citet{rosenbaum1983assessing}, use a latent confounder to evaluate sensitivity binary potential outcomes.  More recently, latent confounder models have been generalized to incorporate more sophisticated potential outcome distributions and non-parameteric regression models \citep{imbens2003sensitivity, mccandless2006, dorie2016flexible}.  Although the latent confounder approach is intuitively appealing, many formulations lead to sensitivity parameters which are \emph{partially identified}.  Partial identification of sensitivity parameters is problematic for three reasons: 1) it leads to a conflation between estimation uncertainty with model ignorance 2) the inferred observed data density depends on the values of the sensitivity parameters and 3) latent confounder models introduce additional computational complexity.  These problems are of practical import.  First, conflating sources of uncertainty can lead to incorrect interpretations and conclusions by investigators.  Furthermore, there is a danger that a given setting of the sensitivity parameters implies a mis-specified observed data model. Finally, because each parameter setting implies a different observed data distributions, the investigator must re-fit the model, with all accompanying computation, for each setting of the sensitivity parameters."} 



%\subsection{Setup}




\subsubsection{Normal Outcome, Binary Confounder}

%it is not generally the case that the sensitivity parameters in a latent confounder formulation are unidentified. The unidentifiability in the Bernoulli   outcome model results directly from the fact that a mixture of Bernoulli random variables is itself a Bernoulli random variable.  Similarly motivated latent confounder models for non-binary potential outcomes often imply sensitivity parameters which are at least partly informed by the data.  



%\avi{Still think we should separate out covariates from no-covariates stuff; this obviously matters for the binary case, will likely matter for Normal case as well}
%\textbf{Binary latent confounder and normal potential outcomes}: 
\citet{imbens2003sensitivity} and \citet{dorie2016flexible} build on the seminal work of \citet{rosenbaum1983assessing} to construct models for normally distributed potential outcomes with unobserved confounders.
We now include observed covariates, $X$, and posit:
%
\begin{align*}
U &\sim \Bern(\pi_u)\\
T \mid U, X &\sim \text{Bern}(g(\beta X + \psi_T U))\\
Y(t) \mid U, X &\sim N(\mu_{Xt} + \psi_Y U, \sigma^2)
\end{align*}
%
\noindent where again $g$ is a link function, e.g., logit or probit function. 
\citet{imbens2003sensitivity} first proposed a linear model for mean of the potential outcomes, $\mu_{Xt} = \tau t + \gamma X$ and \citet{dorie2016flexible} extended the Imbens' approach and models  $\mu_{Xt}$ using Bayesian Adapative Regression Trees.
%As in Equation \ref{eqn:latent_bernoulli_posterior},
We write the conditional distribution of the latent binary confounder $U\mid X, T = \Bern(h(T, X, \pi_u, \alpha, \beta))$.
By Equation \ref{eqn:PO_distribution} we have
%to note the dependence on relevant parameters and observables.  %We can integrate out the binary $U$ 
\begin{align}
\label{eqn:dorie_model}
%U \mid T &= Bern\left(\left[\frac{\pi_U \Phi(\beta X + \phi)}{\pi_U \Phi(\beta X + \phi) + (1-\pi_U) \Phi(\beta X)}\right]^T\right)\\
%U\mid X, T &= Bern(\pi_{uT}(X))\\
Y(t) \mid X, T &\sim h_{\psi_T}(X, T)N(\mu_{Xt} + \psi_Y, \sigma^2) + (1-h_{\psi_T}(X,T))N(\mu_{Xt}, \sigma^2)
\end{align}

In this formulation, the potential outcome distributions are two-component mixture of normal distributions.
The observed and missing potential outcome distributions, $f(Y(t) \mid T = t, X)$ and $f(Y(t) \mid T = 1-t, X)$, respectively, have the same mixture components but different mixture weights.
$\psi_Y$ determines the difference between the component means.
%Here, $\pi_u$ depends on $\psi_Y$ and one of the mixture component means depends on $\phi$.
In this model, the mixture weights, $\pi_{uT}$ and component means are identifiable under relatively weak assumptions \citep[see][]{everitt1985mixture}.  

%``To gain an overall picture of the sensitivity of the treatment effect estimate, we divide the range of valid sensitivity parameters into a grid, and compute b t for each cell of the grid. Valid sensitivity parameters are determined by examining the residual variance after conditioning on observed variables; intuitively, an unmeasured confounder cannot account for any more variability in treatment or outcome than is observed.''  This is a problem because sensitivity parameters informed by data.

\begin{figure}	
	\centering
	\begin{subfigure}[t]{2.5in}
		\centering
		\includegraphics[width=2.0in]{figs/Y0_misspec.pdf}
		\caption{$Y(0) \mid T=0$}\label{y0mis}		
	\end{subfigure}
	\quad
	%\begin{subfigure}[t]{2.5in}
	%	\centering
	%	\includegraphics[width=2.0in]{figs/Y1_misspec.pdf}
	%	\caption{$Y(1) \mid T=1$}\label{y1mis}
	%\end{subfigure}
	\begin{subfigure}[t]{2.5in}
	    \centering
	    \includegraphics[width=2.0in]{figs/pp_bin_norm_plot_1.pdf}
	    \caption{$\pi_{Y^{obs}}(X, 0)$}
    \end{subfigure}
	\caption{Illustrations of partial identification of sensitivity parameters in two sensitivity models, via variation in posterior predictive distributions at different sensitivity parameter settings.
	(a) True (blue) an inferred (red) observed control outcome densities $f(Y(0) \mid T=0)$ (Equation \ref{eqn:dorie_model}) implied by the normal outcome-binary latent confounder model with sensitivity parameters $\psi_T$ and $\psi_Y$. $\Delta \psi_T$ and $\Delta \psi_y$ represent the difference between the true and assumed sensitivity parameters.  The observed data densities are only correctly inferred when we assume the true values of the sensitivity parameters $(i.e. \Delta \psi_T = \Delta \psi_Y = 0$). Note that the true potential outcome distributions $Y(0)$ are a mixture of normals with the same component means and different varainces.
	(b) Posterior predictive expectation functions for observed control outcomes in the binary outcome-normal confounder model with a covariate $X$.
	Solid line shows posterior expectation; shading shows a pointwise 50\% posterior predictive interval.
	When either sensitivity parameter $\psi_T$ or $\psi_{Y0}$ is equal to zero, the surface is monotonic, but when their signs differ, the surface shows non-monotonicity.
	\label{fig:misfit}}
\end{figure}

As a simple demonstration of the implications of partial identification, we simulate data from the normal outcome, binary latent confounder model. As is common practice, we fit the model multiple times for a range of sensitivity parameters.  In Figure \ref{y0mis} we plot the true (blue) and inferred (red) observed potential outcome densities for both potential outcomes.  $\Delta \psi_T$ and $\Delta \psi_Y$ denote the difference between the true and assumed sensitivity parameters.  We have consistent estimates of the observed data only when the assumed values of the sensitivity parameters are the true parameters (i.e. $\Delta \psi_T = \Delta \psi_Y = 0$). 

%It is immediately clear from this formulation that we can expand on the models of \citep{} to the case in which $U$ is a discrete random variable with one of $K$ levels.  In this situation the observed data can be represented as mixture of $K$ components.  


%\avi{explicitly break this apart; how do things change when we incorporate covariates? important point that we're eliding right now}

\subsubsection{Binary Outcome, Normal Confounder}

We follow the same model as above but instead of a binary latent confounder we posit the existence of a normally distributed latent confounder:
%
\begin{align}
U &\sim N(0, 1)\\
%\pi_t &= \Phi \left( \frac{\psi_T}{ \sqrt{1+\psi_T^2} } \right)\\
%f(U \mid T=1) &\propto \phi(U)\Phi(\psi_T + \psi_T U)\\
%\pi_{Y(t)_{\text{obs}}} &= E[g(\beta_t + \psi_Y U) \mid T = t]
T \mid U, X &\sim \Bern(g(\beta X + \psi_T U))\\
Y(t) \mid U, X &\sim \Bern(\pi_{Yt}(X, U))\label{eqn:normalU binary outcome}\\
\pi_{Yt}(X, U) &:= g(\alpha X + \psi_Y U)
\end{align}

Here, given $X$ and $T$, the observed outcome distribution is Bernoulli, and characterized by the function
$$
\pi_{Y^{obs}}(X, T) = \int_{\mathcal U} \pi_{Yt} f(U \mid T, X) dU.
$$

\noindent
%where $f_u(U \mid T)$ is known as the extended skew normal distribution \citep{azzalini2005skew}.
%Again, $\pi_t$ is a continuous monotonic function of $\psi_T$ for any fixed $\alpha$.
%$\alpha$ is not identified from the observed data, but for $\alpha$ fixed to any value, $\psi_T$ is identified.
%Similarly we can use equation \ref{eqn:obs_distribution} to argue that $\pi_{Y(t)_{\text{obs}}}$ is monotonic in $\beta_t$, $\psi_Y$ is completely unidentified and that $\beta_t$ is identified given $\psi_Y$.
In this example, $\mathcal C$ is a smaller family than $\mathcal M$.
In particular, the family $C$ only contains distributions whose mean function $\pi_{Yt}$ is monotone in $X$, given the linear dependence in $\pi_{Yt}$ and the monotonicity of $g$.
Meanwhile, the family $\mathcal M$ contains distributions whose mean function $\pi_{Y^{obs}}(X, T)$ can be non-monotone in $X$ because of the indirect dependence on $X$ introduced by the mixing measure $f(U \mid T, X)$.
This non-monotonicity is particularly pronounced when $\psi_T$ and $\psi_{Yt}$ have opposite sign.



\subsection{Sensitivity Parameter Identification in Latent Confounder Models}

This mixture model perspective is useful for characterizing whether the sensitivity parameters in the latent confounder formulation are identifiable from the observed data distribution.
In particular, we can equate identification of sensitivity parameters to identification of parameters from the mixture $f_\psi(Y^{obs}, T \mid X)$, given by
\begin{align}
f_{\psi_t}(T \mid X) &= \int_{\mathcal U} f_{\psi_T}(T \mid X, U) f(U) dU\\
f^{\rm obs}(Y(t) \mid X, T=t) &= \int_{\mathcal U} f_{\psi_{Y_t}}(Y(t) \mid X, U) f_{\psi_T}(U \mid X, T=t) dU.
\end{align}

Identification in mixture models is a well-studied problem.
\citet{Hennig2000} contains a thorough reference list, with general treatments of the problem given by \citet{teicher1960}, \citet{chandra1977}, and \citet{rao1992}.
\citet{everitt1985mixture} gives an accessible review of identification in the case of finite mixtures.  For our discussion in this section, we focus on partial identification, where the observed data distribution contains information that narrows down potential values for the sensitivity parameters.  We formalize this information in terms of incompatibility between the observed data distribution and the complete data distribution induced by a sensitivity model.

\begin{definition}[Incompatibility]
We say the observed data distribution $f(Y^{obs}, T \mid X)$ is \emph{incompatible} with a sensitivity parameter setting $\tilde \psi$ iff there exists no complete data model $f(Y(0), Y(1), T \mid X)$ with parameters $\tilde \psi$ that induce the true observed data distribution.
\end{definition}

Using this definition of incompatibility, we define partial identification of sensitivity parameters in the latent confounder model.
Let $\mathcal M$ be the family of mixture distributions $f(Y^{obs} \mid T=t, X)$ and let $\mathcal C$ be the family of conditional outcome distributions $f_{\psi_{Yt}}(Y(t) \mid U=u, X)$.
%, and let $\mathcal D$ be the family of latent confounder distributions $f_{\psi_T}(U \mid T)$.

\begin{definition}[Partial Identification of Sensitivity Parameters]
\label{def:partial identification}
The sensitivity parameters $\psi$ in a latent confounder model are partially identified iff there exists some observed outcome distribution $f_m \in \mathcal M$ and sensitivity parameter setting $\tilde \psi := (\tilde \psi_T, \tilde \psi_{Yt})$ such that $f_m$ is incompatible with $\tilde \psi$.
%
%there exists no combination of conditional outcome distributions $f_c \in \{f_{\psi_{Yt}} \in \mathcal C : \psi_{Yt} = \tilde \psi_{Yt}\}$ and mixing measures $f_d \in \{f_{\psi_T} \in \mathcal D : \psi_T = \tilde \psi_T\}$ that satisfy 
%\begin{align}
%f_m(Y^{obs} \mid T, X) = \int_{\mathcal U} f_c(Y^{obs} \mid T, U, X) f_d(U \mid T, X) dU\label{eqn:partial mixture condition}.
%\end{align}
\end{definition}

Here, we show that partial identification occurs under fairly weak conditions on the latent confounder model.
Specific results regarding point identification under more restrictive parametric assumptions are available in the references cited above.
Following \citet{chandra1977}, we state our conditions in terms of the model families of the mixture and conditional outcome distributions.

\begin{proposition}[Sufficient Condition for Partial Identification of Sensitivity Parameters]
\label{prop:partial identification}
Suppose the following two conditions hold:
\begin{itemize}
\item $\mathcal M \supset \mathcal C$, so that the mixture outcome distribution has a strictly larger model family than the conditional outcome distribution, and
\item There exist settings of the sensitivity parameters $\psi$ such that $f_{\psi_{Yt}}(Y(t) \mid U, X)$ does not depend on $U$, or that $f_{\psi_T}(U \mid T)$ is degenerate.
\end{itemize}
Then the sensitivity parameters $\psi$ are partially identified.
\begin{proof}
For any setting of $\psi$ that satisfies the second condition, the corresponding mixture distribution $f(Y^{obs} \mid T, X)$ must lie within $\mathcal C$.
Thus, any mixture distribution $f_m \in \mathcal M \setminus \mathcal C$ is incompatible with these sensitivity parameters, so Definition~\ref{def:partial identification} applies.
\end{proof}
\end{proposition}

\begin{remark}
The case constructed in the proof of Proposition~\ref{prop:partial identification} is particularly important, because it indicates that under the conditions of the theorem, it is possible to reject unconfoundedness based on the observed data on the basis of the parametric specification of the sensitivity model.
\end{remark}

The conditions in Proposition~\ref{prop:partial identification} are weak, but not universal.
The second condition is almost always satisfied by design because it corresponds to having settings of the sensitivity parameters that represent the unconfounded case.
However, the first condition depends on the sample space of $Y^{obs}$ and the parametric specification, and does not hold in some common specifications.
For example, this condition does not hold when $Y^{obs}$ is binary and sensitivity parameters are not shared across covariate strata.
This case includes the classic sensitivity analysis of \citet{rosenbaum1983assessing}, where both outcomes $Y^{obs}$ and latent variable $U$ are binary.
In this case, mixtures of Bernoulli random variables are themselves Bernoulli so $\mathcal M = \mathcal C$.
In fact, we prove in the appendix that the sensitivity parameters in this model are completely unidentified, i.e., there is no partial identification.
%Another example is the case where $f(Y^{obs} \mid T, U, X)$ and $f(U \mid T, X)$ are both normal, $E[Y^{obs} \mid T, U, X]$ is linear in $U$, and sensitivity parameters are not shared between covariate strata; in this case the conditional and mixture distributions of $Y^{obs}$ are normal.
Nonetheless, Proposition~\ref{prop:partial identification} applies in a wide variety latent variables specifications.  In the remainder of this section, we provide examples of partial identification in two models that generalize the sensitivity analysis of \citet{rosenbaum1983assessing}.



%In this work, we are interested in the implications of different latent confounder formulations for the observed outcome densities in the treated and control groups.  These densities have the following form:

%\begin{equation}
%\label{eqn:obs_distribution}
%f(Y(t) \mid X, T=t) = \int f(Y(t) \mid X, U, \theta_t)f(U \mid X, T=t) dU.
%\end{equation}

%and the missing data density has the form

%\begin{equation}
%f(Y(t) \mid X, T=1\-t) = \int f(Y(t) \mid X, U, \theta)f(U \mid X, T=1\-t) \dU
%\end{equation}







==> sections/sec-backup-intro.tex <==
\doublespacing

\section{Introduction}
\label{sec:intro}
%\subsection{Related work}
%Sensitivity analysis plays a central role in observational causal inference.

A fundamental challenge of observational causal inference is that assumptions about unconfoundedness are not testable from data.   Assessing sensitivity to this assumption is therefore important in practice.
Unfortunately, sensitivity analysis is often at odds with modern causal inference approaches, especially those that use nonparametric techniques to build highly flexible models of the observed data.
For example, several recent approaches rely on Bayesian nonparametric or other machine learning methods to flexibly model the outcome surfaces under unconfoundedness \citep{hill2012, athey2017, hahn2017bayesian}. 
In many cases, however, incorporating sensitivity analysis into these models has unintended consequences: perturbing both the unobservable influence of the confounders (as planned) \emph{and} the observable predictions of the model (not as planned). This degrades the quality of observed data predictions and introduces other unnecessary complications. 
 
In this paper, we explore an alternative sensitivity analysis framework that resolves this tension and allows for incorporating flexible, nonparametric methods into model-based sensitivity analysis. 
% We do so by applying a particular factorization from the missing data literature, known as the \emph{extrapolation factorization}. 
We focus on a particular observed data parameterization called the \emph{extrapolation factorization}.  For univariate missing data, the joint distribution factors in terms of the observed data density, which is nonparametrically identified, and the selection function, which is unidentified but easily interpreted.  Given a specification for the unidentified selection functions, complete inference proceeds by extrapolating the missing data distributions from the observed data distributions.  The extrapolation approach was first introduced by John Tukey for univariate missing data \citep[recorded in][]{holland-notes}, which he termed the ``simplified selection model,'' 
% This approach combines elements of both the selection factorization and pattern-mixture factorization 
and has more recently been used under different names including exponential tilting \citep{Birmingham2003, Scharfstein1999}, Tukey's factorization \citep{franks2016non},  and the extrapolation factorization \citep{linero2017bayesian}.  

Our main contribution is to apply the extrapolation factorization to assessing sensitivity to unconfoundedness in observational studies. To the best of our knowledge, this is the first thorough demonstration of its use for this application, which leads to several gains in practice.
% The extrapolation factorization has several advantages over existing approaches.  
%
First, this approach enables separate quantification of the sensitivity of the results to both changes in the observed data model (testable) and sensitivity parameters (untestable).  Perturbations to a ``true'' sensitivity parameter should not be testable from the observed data  \citep{linero2017bayesian, gustafson2018sensitivity} and so by separating observable and unobservable implications, we resolve a common conflation between sensitivity analysis and model selection.  An important consequence of this separation is that the framework can easily be used for \emph{any} probabilistic predictive model, allowing investigators to add sensitivity analysis to a causal investigation regardless of the statistical model.  We demonstrate this flexibility by conducting sensitivity analysis with a range of modern statistical models including Bayesian Adapative Regression Trees (BART) for response surface estimation \citep{dorie2016flexible} and Dirichlet processes models for non-parametric inference of residual distributions.  We also demonstrate the use of the factorization with semi-continuous data using zero-inflated models.  

Second, for a sensitivity analysis to be meaningful, the sensitivity parameters must be interpretable. A factorization that explicitly incorporates the selection function facilitates both interpretable model specification and improved parameter calibration. This is a major advantage over traditional pattern-mixture models which do not explicitly parameterize the selection function.  


Third, in this factorization, observed data inference is orthogonal to the specification of the selection function, which yields a straightforward framework for conducting \emph{post facto} sensitivity analysis in any data set for which unconfoundedness was previously assumed. This fact implies substantial computational savings because we only need to fit a model to the observed data once. In contrast, with complete data models, we typically need to fit the model separately for each set of sensitivity parameters. 


The paper proceeds as follows.
Section \ref{sec:setup} introduces the formal setup for sensitivity analysis and highlights key issues.
Section \ref{sec:latent-confounder} discusses the difficulties of complete data modeling in causal inference, in particular by studying a common class of models known as  \emph{latent confounder models}.  Here, we demonstrate how some standard specifications lead to sensitivity parameters that are at least partially identified. 
Section \ref{sec:tukey_causal} introduces the extrapolation factorization for causal inference and provides theoretical justification for applying the approach. 
Section \ref{sec:example_specs} defines a particular model specification, the logistic-exponential family model, and explores implementation details. 
Section \ref{sec:analysis} applies the extrapolation factorization to two examples, demonstrating the flexibility of the approach on a range of estimands with several Bayesian nonparametric estimation approaches.
%Section \ref{sec:mix-model} discusses an alternative specification for the extrapolation factorization based on a mixture model representation that is closely related to the latent confounder approaches.
Finally, Section \ref{sec:discussion} discusses open issues and possible extensions. The appendix contains some additional technical material.











\section{Setup and Outline} 
\label{sec:setup}

% \damour{Things that need to be defined earlier: \st{unconfoundedness and overlap}, \st{population-level estimand}, ignorance and uncertainty regions, are the estimates in the latent confounder model valid causal effects, specification testing vs sensitivity analysis.}

\subsection{Setting and Notation}

We describe our approach using the potential outcomes framework \citep{neyman1923, rubin1974}. For outcome $Y_i$ for unit $i$, let $Y_i(0)$ and $Y_i(1)$ denote that unit's potential outcomes if assigned to control or treatment, respectively. We let $T_i$ denote a binary treatment indicator and $X_i$ denote observed covariates. For compactness, we often write $Y_i(t),\: t \in \{0, 1\}$ to denote the outcome for treatment level $t$. Assuming SUTVA \citep{rubin1980comment}, we can then write the observed outcome as:
$$
Y_i^{\text{obs}} =: T_i Y_i(1) + (1-T_i) Y_i(0).
$$
with corresponding density $f^{\rm obs}(Y_i(t) \mid T_i = t)$. Finally, we write the propensity score as
$
e(x) = P(T_i = 1 \mid X_i = x).
$
We assume an infinite population of iid units, from which we sample triplets $([Y_i(0), Y_i(1)], T_i, X_i)$ and observe triplets $(Y^{\text{obs}}_i, T_i, X_i)$. Given this, we suppress the subscript $i$ unless otherwise noted.



We focus on two classes of population estimands.
First, we consider average treatment effects on the whole population as well as on the treated and control populations:
\begin{align*}
\tau^{ATE} &:= E[Y(1) - Y(0)] = E[Y(1)] - E[Y(0)]\\
\tau^{ATT} &:= E[Y(1) - Y(0) \mid T = 1] = E[Y(1) \mid T = 1] - E[Y(0) \mid T = 1]\\
\tau^{ATC} &:= E[Y(1) - Y(0) \mid T = 0] = E[Y(1) \mid T = 0] - E[Y(0) \mid T = 0].
\end{align*}
Secondly, we consider quantile treatment effects,  $$\tau_q =  Q_q(Y(1)) - Q_q(Y(0))$$
\noindent the difference in the $q$-th treatment quantile, $Q_q(Y(1))$, and control quantile, $Q_q(Y(0))$.









%%%
%%% OVERVIEW OF SENSITIVITY
%%%
\subsection{Sensitivity Analysis Overview}

%\avi{Put in overview of our approach here; if unconfoundedness holds, then $f^{mis} = f^{obs}$; otherwise, they ain't}


We consider sensitivity analyses for observational studies where the investigator wishes to test robustness to violations of the unconfoundedness assumption.
\begin{assumption}[Unconfoundedness]
\label{assn:unconfounded}
$[Y(0), Y(1)] \independent T \mid X $.% for $t = 0, 1$.
\end{assumption}

%The primary assumption made regarding $f^{mis}$ is unconfoundedness, which implies that $f^{mis}$ = $f^{obs}$.
%We consider sensitivity analyses for observational studies where the investigator wishes to test robustness to violations of the unconfoundedness assumption.

There is an extensive literature on assessing sensitivity to departures from unconfoundedness, dating back at least to the foundational work of \citet{cornfield1959smoking} on the link between smoking and lung cancer. 
% we address only the small portion of that literature that uses likelihood-based (or model-based) sensitivity analysis, largely built on \citet{rosenbaum1983assessing}.
In this paper, we focus on model-based sensitivity analysis, which proceeds by specifying a family of models for the joint distribution of potential outcomes and treatment given covariates.
% , with density $f([Y(0), Y(1)], T \mid X)$. 
% This is often in the spirit of \citet{rosenbaum1983assessing}, who specify a binary latent confounder in settings with a binary outcome.
% Although it can be challenging to fully specify such a model, it can be used to simultaneously estimate \emph{any} estimands that are functions of the complete data, including continuously indexed estimands, e.g., quantile treatment effects $\tau_q$.
% Since new analyses are not needed for estimating different estimands, likelihood-based methods can easily be applied to a very general class of problems.
For distinct approaches to sensitivity analysis, see~\citet{rosenbaum2009amplification}, ~\citet{ding2016sensitivity}, and \citet{zhao2017sensitivity}.

In a model-based sensitivity analysis, the investigator typically proceeds by specifying a family of missing potential outcome distributions that represents a set of plausible departures from unconfoundedness.  Here, given unobserved confounding, we parameterize the conditional dependence between partially-observable potential outcomes $[Y(1), Y(0)]$ and $T$ given covariates $X$. 
The parameters of this dependence are called \emph{sensitivity parameters}.
Investigators can then report how causal effect estimates change when the sensitivity parameters are allowed to vary within a selected range of plausible values.
The plausibility of the range of sensitivity parameters is ultimately determined externally to the data analysis, e.g., by domain expertise.

Broadly, there are two approaches to model-based sensitivity analysis, \emph{complete} data modeling and \emph{observed} data modeling; both have been thoroughly explored in the missing data literature \citep{van-buuren2015aa} but are perhaps less studied in causal inference. 
Complete data modeling, also known as the selection factorization, is the standard approach for model-based sensitivity analysis in causal inference \citep{rosenbaum1983assessing, dorie2016flexible}. These models factorize the joint distribution of outcomes and missingness indicators into the product of the marginal distribution of the outcome and the conditional distribution of the missingness indicator given the outcome \citep{rubin1974aa}. 
% This approach is the standard factorization for model-based sensitivity analysis in causal inference \citep{dorie2016flexible}. %
In this paper we utilize a third approach, also stemming from the missing data literature termed the extrapolation factorization.  For some sensitivity parameter $\psi$, let $f^{\rm mis}_\psi(Y(t) \mid T = 1\-t, X)$ be the unidentified missing data density in treatment arm $t$.  
The key to the approach used in this paper, is that we implicitly parameterize $f^{mis}_{t,\psi}$ by defining a complete-data model 
$f\psi([Y(t), Y(1-t)], T \mid X)$ for which the missing potential outcome distributions are defined via an extrapolation of the observed data: $f^{\rm mis}(Y(t) \mid T=1\-t, X) \propto \frac{f_\psi(T=t\mid Y(t), X)}{f_\psi(T=1\-t\mid Y(t), X)}f^{\rm obs}(Y(t) \mid T=t, X)$.  This factorization makes it clear that only when $f_\psi(T \mid Y(t), X) = f_\psi(T \mid X)$ is the missing data density identified from the observed data, e.g. unconfoundedness holds and $f^{\rm mis}(Y(t) \mid T=1\-t, X) = f^{\rm obs}(Y(t) \mid T=t, X)$.  This factorization has clear advantages over complete data models as well as over other observed data factorizations like the pattern mixture factorization \citep{Rubin1977,little1993}.  We introduce this factorization for causal inference formally in Section \ref{sec:tukey_causal}.  

Sensitivity analyses often involve two key design choices that are easily addressed by our approach. First, the analyst faces many choices in modeling the conditional dependence between outcomes and treatment.  Our approach follows recent proposals to enable sensitivity analysis with flexible outcome models, especially ~\citet{dorie2016flexible}, who use Bayesian Additive Regression Trees (BART) models for flexible outcome modeling \citep[see also][]{carnegie2016assessing}. We contrast their approach with ours in Section \ref{sec:analysis_nhanes}. Similarly, \citet{jung2018algorithmic} combine flexible, black-box modeling with sensitivity in the setting of algorithmic decision making. As we discuss in Section \ref{sec:latent-confounder}, our main critique has limited applicability to their approach, since \citet{jung2018algorithmic} focus exclusively on the setting with a binary outcome and sensitivity parameters that vary across covariates.
Finally, in an approach that aligns well with ours, \citet{hahn2016bayesian} propose flexible, nonparametric models that separate the observed data model from sensitivity parameters in the context of missing data.

Second, the analyst must summarize the results of the sensitivity analysis. Setting the range of sensitivity parameters is a critical first step; it can be useful to calibrate this range against similar measures of dependence between fully observed variables, e.g., $T$ and $X$ \citep{imbens2003sensitivity, ichino2008temporary, dorie2016flexible}.
In some literatures, the range of causal estimates obtained by allowing sensitivity parameters to vary within the specified range is called an \emph{ignorance region}, and we adopt this terminology in this paper \citep{Vansteelandt_Ignorance_2006}.
For ignorance region reporting, we focus on what is sometimes called the ``tabular method'', where we evaluate causal effect estimates across a grid of sensitivity parameter values \citep{gustafson2018sensitivity}, and report the entire table of estimates.
Our methodology is not restricted to this type of reporting, but we find it useful to demonstrate several important properties of our sensitivity analysis framework, including the non-identification of sensitivity parameters.
Alternatives to the tabular method include so-called Bayesian sensitivity analysis, where the investigator specifies a prior over sensitivity parameters and reports a posterior on treatment effects given the full model \citep{mccandless2007bayesian,mccandless2017comparison}, and bound reporting, where the investigator simply reports the most extreme causal effect estimates obtained from sensitivity parameters within the specified range \citep{Rosenbaum_Observation_2017}.
One disadvantage of the tabular method is that it is only feasible to do this reporting with low-dimensional sensitivity parameters.



% \subsection{Sensitivity Analysis as Missing Outcome Specification}

% \damour{Some fragments of what I wrote...}

% Sensitivity analysis plays a central role in causal inference because the distribution of missing outcomes is unidentified.
% As a result, causal estimands that are defined as contrasts between observed and missing outcome distributions are only identified under untestable assumptions about the missing outcome distributions.
% % For example, when estimating the ATT while adjusting for $X$, we contrast the expectation implied by $f^{\textrm{obs}}_1 = f(Y(1) \mid T = 1, X)$ with the expectation implied by $f^{\textrm{mis}}_0 = (Y(0) \mid T = 1, X)$.
% % Here, $f^{\textrm{obs}}_1$ is nonparametrically identified by the observed data, while $f^{\textrm{mis}}_0$ factor is completely uninformed.
% % Thus, in principle, any distribution $f^{\textrm{mis}}_0$ on the support of $Y$ would be compatible with the observed data, along with the ATT implied by $f^{\textrm{mis}}_0$.
% Note that unconfoundedness resolves this ambiguity by setting $f^{\textrm{mis}}_0 = f(Y(0) \mid T = 0, X)$.




\subsection{Separating Sensitivity Analysis from Model Checking}

A prime motivation for our sensitivity analysis framework is that it enforces a clean separation between sensitivity analysis and model checking.
Model checking probes observable parts of the model and explores a range of assumptions that induce distinct models for the observed data.
Sensitivity analysis, by contrast, probes \emph{unobservable} parts of the model and explores the range of causal conclusions that are compatible with a fixed model of the observed data. 
Both sensitivity analysis and model checking are essential parts of causal inference, but it is necessary to distinguish between them.

%Each type of perturbation answers a different question and each type of ambiguity suggests a different response for resolution.

%The ambiguity sensitivity analysis can only be resolved by bringing in external information, whether that be data produced under a different design, or prior knowledge about the data generating process under study.  
In practice, however, many popular approaches to sensitivity analysis blur the line between sensitivity analysis and model checking by introducing sensitivity parameters that are identified by the observed data.
Sensitivity analyses of this type are difficult to interpret because they deal with two interacting sets of assumptions at once.
Specifically, they relax the unconfoundedness assumption while introducing parametric assumptions that fundamentally change the relationship between confounding and identification.
This creates new types of sensitivity that go unexamined by the analysis itself.
For example, under some parametric models for complete data, the unconfoundedness assumption, which has no observable implications on its own, becomes testable.
%The presence of identified sensitivity parameters implies that the sensitivity model incorporates additional parametric assumptions that fundamentally change the relationship between confounding and identification.
%In such a case, the sensitivity parameters specify a range of distinct observed data models, rather than specifying a range of causal interpretations compatible with a single observed data model.
%When a sensitivity analysis includes identified sensitivity parameters, it implies that the sensitivity model has introduced additional identifying assumptions at the same time that it has relaxed the unconfoundedness assumption.
In the context of missing data, \citet{linero2017bayesian} describe a detailed case, due to \citet{Kenward_Selection_1998}, where slight changes in the tail thickness of a parametric complete-data model specification result in different test-based conclusions about ignorability.

Conflating model checking with sensitivity analysis also has practical implications.
First, sensitivity analysis with identified sensitivity parameters is computationally expensive because each setting of the sensitivity parameters requires that the model be re-fit \citep{hahn2016bayesian}.
This is particularly onerous when a sensitivity analysis strategy is employed with modern nonparametric strategies that are relatively expensive to fit.
Second, exploring a range of distinct model fits in a \emph{post hoc} sensitivity analysis raises the spectre of data snooping.
As opposed to a valid sensitivity analysis, where the investigator could tune an observed data model in a held-out sample, in a sensitivity analysis with identified sensitivity parameters, the investigator could choose the model fit that is the most favorable to their conclusions and declare it to be the ``main'' model whose robustness is being checked  \citep[][p. 172, ``What Is Not a Sensitivity Analysis?'']{Rosenbaum_Observation_2017}.
Finally, \citet{gustafson2018sensitivity} note that identified sensitivity parameters often introduce ``funny business'' when the prior information used to calibrate the sensitivity parameters ends up in competition with the observed data.

For these reasons, we prioritize separation of sensitivity analysis and model checking in this paper. We do this by proposing a sensitivity analysis framework that fixes the observed-data model. 
This represents a point of departure from some popular complete-data sensitivity analysis frameworks for causal inference, where it can be difficult to specify unidentified sensitivity parameters.  We describe these difficulties below.  

%For binary potential outcomes the odds ratio is also sometimes of interest:
%
%$$ \tau^{OR} = \frac{p_1}{1-p_1} / \frac{p_1}{1-p_0}$$
%
%with $E[Y(0)] = p_0$ and $E[Y(1)] = p_1$.  






%We provide examples of sensitivity analysis with Bayesian nonparametric models including Dirichlet Process mixture models and  Bayesian Additive Regression Trees.

% \subsection{Refs to incorporate}
% \begin{itemize}
% \item \citep{rosenbaum2002covariance} 
% \item \citep{keele2010overview} 
% \item \citep{cinelli2018making}
% \item \citep{dorie2016flexible} 
% \item \citep{zhao2017sensitivity} 
% \item \citep{riddles2016propensity} 
% \item \citep{imbens2003sensitivity}  
% \item \citep{gustafson2018sensitivity} 
% \item \citep{mccandless2006} 
% \item \citep{xu2018bayesian}
% \end{itemize}

%Extrapolation factorization.  In Section \ref{sec:tukey_causal} we introduce the extrapolation factorization for assessing sensitivity to unobserved confounders in causal inference.  

%\avi{This is short enough that I think we should move it up to an earlier lit review; not sure it really belongs here, plus it's nice to motivate the different factorizations earlier, I think; also gives us a chance to talk about what's different (if anything) with causal stuff}




%In this section, we demonstrate the implications of different latent confounder formulations on the fit of the observed data distribution. Specifically, we show that, in many practical cases, the sensitivity parameters are partially identified (and/or that the observed data density depends on the sensitivity parameters). This matters more for continuous outcomes.


%\section{Likelihood-Based Sensitivity Analysis}
%\label{sec-missing-data}

%\damour{Fold the lit review into this section?} \avi{Prob a good idea. Useful to differentiae likelihood-based sensitivity analysis from other approaches. Most obvious alternatives are (1) moment-based approaches, like Cornfield conditions/Peng's stuff; and (2) single-parameter approaches like Rosenbaum's, which implicitly rely on a likelihood, but not as explicitly as R\&R}

%In this section we briefly review the literature on modeling \emph{univariate} non-ignorable missing data, before describing an application of a particular approach, the extrapolation factorization, to causal inference. 















%However, Equation \ref{eqn:miss} makes it clear that this factorization can only be used when the observed and missing data densities have common support.  \citet{franks2016non} show that in practice the extrapolation factorization should be used cautiously when the observed data density is very small in places where the missing density is very large, as results can be very sensitive to estimates of the observed data in low-density regions.  %In the next section we show how the extrapolation factorization can be applied to applications in causal inference.














% \section{Models for non-ignorable missing data}
%\subsection{Related methods}


%As described above, by integrating out the latent confounder, we can identify the implications for the observed and missing data distributions. In this paper, we do not explicitly model dependence on a latent confounding variable.  Rather, our approach is to directly model the triplet $(T_i, [Y_i(0), Y_i(1)] \mid X_i)$.  If $X_i$ is not sufficient for unconfoundedness then, $T_i \text{ }\cancel{\independent}\text{ } [Y_i(0), Y_i(1)] \mid X_i$.  Thus, all models under confoundedness must include some specification for the dependence between $T_i$ and $Y_i$.  %In this section we briefly review the literature on modeling \emph{univariate} non-ignorable missing data, before describing an application of a particular approach, the extrapolation factorization, to causal inference.  

% In what follows, we suppress conditioning on $X_i$ for notational clarity.

% \newline
% \newline

% \noindent \textbf{The selection factorization:} 
% \subsection{Missing Data Factorizations}

%In the selection factorization approach \citep{rubin1974aa}, the joint distribution, $(Y_i,T_i)$, is factorized into a the distribution for the complete data, $P(Y|\theta_Y)$, and the missingness mechanism, (or selection function), $P(T|Y,\theta_{T|Y})$.  Specifically, we posit
%$$P(Y,T \mid \theta) = \prod_i^N f(Y_i|\theta_Y)f(T_i|Y_i,\theta_{T|Y})$$
%
%A common alternative is the pattern-mixture approach \citep{Rubin1977,little1993}.  The pattern-mixture formulation decomposes the joint distribution into a mixture of observed
%data and missing-data components.  This factorization leads to a mixture likelihood, which for the complete data density of single  observation is
%$$ P(Y_i \mid \theta) = \sum_{t=0}^1 f(T_i=t|\theta_T).f(Y_i|T_i=t, \theta_{Y|tT=t})$$
%
%where $\theta = (\theta_{Y|T=1}, \theta_{Y|T=0}, \theta_T)$ are the observed data parameters, missing data parameters, and the population fraction of missing data respectively.
%That is 
%$$f(Y_i,T_i | \theta) &=& f(Y_i|T_i, \theta_{Y|T})f(T_i|\theta_T) = \left[f(Y_i|T_i=r, \theta_{Y|T=t})f(T_i=t|\theta_T)\right]^{I(T_i=t)}$$, where $\theta = (\theta_{Y|T=1}, \theta_{Y|T=0}, \theta_T)$ are the observed data parameters, missing data parameters, and the population fraction of missing data respectively. 
%
%The selection factorization is commonly, and under certain parametric assumptions leads to identification of the $\theta_Y$ and $\theta_{T|Y}$ \citep{linero2017bayesian}. Importantly, neither $\theta_Y$ or $\theta_{T\mid Y}$ are individually identifiable, but under certain parametric assumptions they can jointly be identified (see \avi{cite}).  We argue that this is problematic in many settings, including causal inference, since this factorization mixes the identifiable component (parameters governing the observed data density) with the unidentifiable ones (the form of the non-ignorability).  Specifically, the implied observed data density depends on both $\theta_Y$ and $\theta_{T|Y}$ which means that not all values of the sensitivity parameters are equally likely for a given set of observed data.


%In contrast, the pattern mixture factorization explicitly issues associated with the selection factorization at the expense of interpretability. Notice that we model the observed and missing data densities directly, thus completely separating the identifiable and unidentifiable components of the model. However, the major downside to this approach is that we rarely have any direct intuition or prior knowledge about the missing data density.  In particular, the selection function $f(T_i \mid Y_i, \theta_{T|Y})$, which is typically easier to think about, is not specified at all in this factorization.  In the following section, we describe the extrapolation factorization which we argue combines the benefits of both the selection and pattern-mixture factorizations.  

%\subsection{Joint sensitivity model}
%\avi{I think this is the standard latent variable formulation where $U$ affects both $T$ and $Y$}

==> sections/sec-example-specs.tex <==
\section{Logistic Model Specifications}
\label{sec:example_specs}
In the previous section, we showed that, to conduct sensitivity analysis for many common  causal estimands like the ATE and QTE, it is sufficient to supplement the observed data model with a specification of unidentified marginal selection functions $f(T \mid Y(t), X), t \in \{0, 1\}$.
%, in addition to the fully identified the marginal observed data densities, $f(Y(t) \mid T=t, X)$.%  Although there are infinitely many ways to specify the unidentified selection functions, for sensitivity analysis to be practically applicable, the models should involve a small number of \emph{interpretable} sensitivity parameters and be computationally tractable.
%Each model borrows elements that are common in the latent confounder models discussed in Section \ref{sec:latent-confounder}.  
%: the logistic-EF formulation and the mixture-selection formulation.  In the logistic-EF formulation, the selection function is assumed to be logistic and the observed data an exponential family distribution.  The sensitivity parameters have simple interpretations, and as shown, can be easily incorporated into nonparametric models by applying our results to mixtures of exponential families.  We also proposed the mixture-selection function for situations in which the observed data distribution is best modeled as a mixture of two latent classes. 
%
% In principle, the models for the selection functions and the observed data densities can all be specified independently, but in practice there are practical advantages to choosing selection models and observed data models that work well together. In particular, in this section we describe classes of models that are computationally tractable, facilitate parameter calibration and interpretation, and which further elucidate the benefits of the extrapolation factorization. 
%\avi{I like this paragraph, but the intro to this section is now too long... maybe we keep for now and cut later?} 
%
% In Section \ref{sec:logit-ef}, we explore sensitivity analysis with 
In this section, we propose a simple class of marginal selection function using a logistic specification.
Specifically, we posit that the log-odds of receiving treatment are linear in some sufficient statistics of the potential outcomes, $s(Y(t))$:
\begin{align}
\label{eqn:logistic selection}
f(T = 1 \mid Y(t), X) &= \text{logit}^{-1}\hbox{}\{\alpha_t(X) + \gamma_t' s_t(Y(t))\},
\end{align}
where $\text{logit}^{-1}\hbox{}(x) = (1 + \exp(-x))^{-1}$.
This specification has sensitivity parameters $\gamma = (\gamma_0, \gamma_1)$, which separately describe the sampling bias among control and treated units, respectively.
Logistic selection is commonly used in latent confounder approaches to model the probability of treatment given the unobserved confounder.
Here, we take a similar approach, but assume that the treatment probabilities are logistic in sufficient statistics of the potential outcomes.
We demonstrate the properties of extrapolations implied by logistic selection models, then discuss some strategies for interpreting and calibrating the sensitivity parameters in this specification.
% We provide simple examples for binomial, normal and mixture-of-normal distributions.  %In Section \ref{sec:mix-model} we introduce an alternative model for causal sensitivity analysis motivated by the binary latent confounder models introduced in Section \ref{sec:latent-confounder} (e.g. example 1), but for which the sensitivity parameters are not identified.  We show that in this latent class specification, the selection function is not logistic, but rather has selection probabilities that asymptote at values strictly between 0 and 1. In particular, unlike the logistic-EF class, the latent class approach implies a bounded ignorance region for treatment effects.  
% In Section \ref{sec:calibration} we describe parameter interpretation and provide approaches for sensitivity parameter calibration in the class of logistic models. 
%In Section \ref{sec:mix-model}, we suggest an alternative family of models based on a latent class formulation.

%We illustrated the flexibility of these models by computing quantile treatment effects on a grid of quantiles, under different assumptions about unconfoundedness.  We also showed how these models can be applied to a range of data sets including non-parametrically estimated mixture models and zero-inflated data.

\damour{How useful is it to define the notion of ``logistic EF'' models as a thing vs logistic selection with exponential family observed data models?}

\subsection{Logistic Selection with Exponential Family Models}
\label{sec:logit-ef}

In this section, we explore some of the properties of the extrapolations implied by logistic selection functions when the observed data distribution is a member of the exponential family, or is a mixture of exponential family distributions. 
Following \citet{franks2016non}, we show that with observed data distributions of this form, logistic selection functions induce analytical extrapolations.
%In the logistic-EF models, we assume that the observed data distributions, $f^{\rm obs}(Y(t)\mid T=t, X)$, can be modeled using a mixture of exponential family distributions and that the logit of the selection mechanisms, $\text{logit}(f(T \mid Y(t), X))$, is linear in the sufficient statistics of the exponential family.
Logistic selection functions can be applied more broadly than to this class of models, but we note that mixtures of exponential families are a flexible model class, and include non-parametric methods like Dirichlet process mixtures.
Thus, beyond being convenient analytical examples, the results in this section can be used directly to efficiently implement sensitivity analysis with many flexible observed data models. 
%This approach is quite general, since we can apply the extrapolation factorization to observed data densities modeled with non-parametric methods like Dirichlet process mixtures.
%Further, the logistic selection function is commonly used in causal inference and can easily be interpreted.
\paragraph{Single exponential family models.}
We start by describing the extrapolations of observed data densities that belong to a single exponential family distribution and later describe the extension to mixtures.  Here, we model the observed data as an exponential family distribution with natural parameter $\eta_t(X)$, possibly depending on $X$, 
%
\begin{equation}
\label{eq:exp-log-obs}
f^{\rm obs}_{\eta_t}(Y(t) \mid, T=t) = h(Y(t))g(\eta_t)e^{s(Y(t)) ' \eta_t(X)}
\end{equation}
%
where $g(\eta_t)$ is the partition function, $h(Y(t))$ is the base measure and $s(Y(t))$ is the natural sufficient statistic, possibly multivariate, for the exponential family.
%
%
%\begin{equation}
%\label{eq:exp-log-sel}
%f_{\gamma_t}(T = t \mid Y(t), X) = \text{logit}^{-1}\hbox{ }(s(Y(t))\gamma_t + \mu_t(X)) = \frac{1}{1+e^{-s(Y(t))'\gamma_t + \mu_t(X)}}
%\end{equation}
%
%This implies that
%
%\begin{equation}
%\nonumber \frac{f(T = t \mid Y(t), X)}{f(T = 1\- t \mid Y(t), \gamma_t)} = e^{- s(Y(t))'\gamma_t)}
%\end{equation}
%
When selection function is assumed to have form \eqref{eqn:logistic selection}, 
\citet{franks2016non} show that
%for the class of exponential-logistic models defined by Equations \ref{eq:exp-log-obs}--\ref{eq:exp-log-sel},
the missing data distribution belongs to the same exponential family as the observed data, with natural parameter $\eta^*_t(X) = \eta_t(X) + \gamma_t$,
%
\begin{equation}
\label{miss_dist_ef}
f^{\rm mis}_{\eta_t, \gamma_t}(Y(t) \mid T = 1-t) = h(Y(t)) g(\eta^*_t) e^{{s(Y(t))}'\eta^*_t(X))}
\end{equation}
%
\noindent The implied complete data density $f_{\eta_t, \gamma_t}(Y(t))$ can then be expressed as a simple mixture of the observed and missing components.  In this specification $\gamma_t$ are sensitivity parameters that independently parameterize sensitivity for the control and treated groups. Importantly, the sensitivity parameters are independent of the covariates. We return to this point in the discussion.
%
% \avi{Fix after this; cross-check with discussion at end} Further, sensitivity to unobserved confounders does not vary with covariates.  This is because the $\gamma_t$ does not covary with $X$ and enters the selection function additively. An important consequence of this fact is that $\mu_t(X)$ does not influence causal estimands \footnote{Although $\mu_t(X)$ does not influence causal estimates, estimates of this quantity can still be useful for calibrating $\gamma_t$ (See Section \ref{sec:calibration})}.  In theory, we can allow for richer parameterizations in which the strength of the non-ignorable selection varies with $X$, but at the cost of interpretability and computation. We revisit this in the discussion. 
%
To provide some intuition for how extrapolation operates under this specification, we present two simple examples.
%about the extrapolation factorization, we briefly discuss three examples of increasing complexity for different parametric observed data specifications.

\begin{example}[Binary potential outcomes]  Let $Y(t) \in \{0, 1\}$ and
%
\begin{align*}
f^{\rm obs}(Y(t) \mid T=t, X) &\sim \Bern(\text{Logit}^{-1}(\mu_t(X))\\
f(T \mid X, Y(t)) &\propto \Bern(\text{Logit}^{-1}(\alpha_t(X) + \gamma_t Y(t)))
\end{align*} 
%
\noindent By Equation \ref{miss_dist_ef} the unobserved potential outcome distribution is:
%
\begin{align*}
f^{\rm mis}(Y(t) \mid T=1\-t, X) &\sim \text{Bern}(\text{Logit}^{-1}(\mu_t(X) + \gamma_t))
\end{align*}
%
\noindent Thus, the extrapolation factorization with logistic treatment assignment applied to Bernoulli data implies an additive shift in the log-odds of the unobserved potential outcomes (relative to the observed potential outcome distribution).
\end{example}

\begin{example}[Gaussian potential outcomes] Because the normal distribution is a two parameter exponential family distribution with sufficient statistics $s(Y(t) = (Y(t), Y(t)^2)$, we consider a treatment assignment mechanism that is quadratic in the potential outcomes. 
%
\begin{align*}
f^{\rm obs}(Y(t) \mid T=t, X) &\sim \text{Normal}(\mu_t(X), \sigma_t^2)\\
f(T \mid Y(t)) &\propto \text{Bern}(\text{Logit}^{-1}(\alpha_t(X) + \gamma_t Y(t) + \psi_tY(t)^2))
\end{align*} 
%
\noindent By Equation \ref{miss_dist_ef} the unobserved potential outcome distribution is:
%
\begin{align}
\label{eqn:norm_example_mis}
f^{\rm mis}(Y(t) \mid T=1\-t, X) &\sim \text{Normal}\left(\frac{\mu_t(X) + \gamma_t\sigma_t^2}{1 - 2\psi_t\sigma_t^2} , \frac{\sigma_t^2}{1 - 2\psi_t\sigma_t^2}\right)
\end{align}
%
This model has two sensitivity parameters for each treatment arm. Assuming that the logistic function is linear in $Y(t)$, i.e. $\psi_t=0$, implies that standard deviations of observed and missing potential outcome distributions are identical.\footnote{Note that in the quadratic model we require $\psi_t > \frac{1}{2\sigma_t^2}$ to ensure propriety of the missing potential outcome distribution.}
In Section \ref{sec:analysis_nhanes} we conduct a sensitivity analysis on potential outcomes with flexibly estimated response surfaces, by estimating $\mu_t(X)$ from the observed data using BART.
\end{example}

\paragraph{Mixtures of exponential families.}
Logistic extrapolations of exponential family models are easily extended to mixtures of exponential family distributions.
%The logit-EF formulation can easily be extended to mixtures of exponential families.
Let $f^{\rm obs}(Y(t) \mid \eta_t, T=t) = \sum_k \pi_k h_k(Y(t))g_k(\eta_{tk})e^{s(Y(t)) ' \eta_{tk}}$ be a mixture of exponential family distributions with mixture weights $\pi_k$.  Then, as shown in \citet{franks2016non},
%
\begin{align}
\label{eqn:ef_mix_miss}
f^{\rm mis}(Y(t) \mid \eta_t, \gamma_t, T=1-t) = \sum_k \pi^*_k h_k(Y(t))g_k(\eta^*_{tk})e^{s(Y(t)) ' \eta^*_{tk}}
\end{align}
%
where $\eta^*_{tk} = \eta_{tk} + \gamma_t$, as above, and
%
\begin{align}
\label{eqn:ef_mix_weights}
\pi_k^* &= \frac{\pi_k\frac{g(\eta_k)}{g(\eta_k^*)}}{\sum_k^K
        \pi_k\frac{g(\eta_k)}{g(\eta_k^*)}}
\end{align}
Consider the following simple example.
%

\begin{example}[Gaussian mixture potential outcomes]
As a simple example, we extend the normal model above to a finite mixture of normal distributions: $f^{\rm obs}(Y(t) \mid T=t, X) \sim \sum^K \pi_k \text{Normal}(\mu_{tk}(X), \sigma_{tk}^2)$.
%and $f(T \mid Y(t), X) = \text{logit}^{-1}(\alpha_t(X) + s(Y(t))'\gamma_t) $.  
For simplicity we assume $\psi_t = 0$.  Then, by Equations \ref{eqn:ef_mix_miss} and \ref{eqn:ef_mix_weights}, %\avi{$1-t$ in the conditioning set?}
\begin{align}
\label{eqn:mix_normal_dists}
f^{\rm mis}(Y(t) \mid T=1-t, X) &\sim \sum \pi^*_k \text{Normal}(\mu_{tk}(X) + \gamma_t\sigma_{tk}^2, \sigma_{tk}^2)\\
\pi^*_k &\propto \pi_k \exp\frac{1}{2}\left({\frac{\mu_{tk}^2(X)}{\sigma_{tk}^2} - \left(\frac{\mu_{tk}(X)}{\sigma_{tk}} - \gamma_t\right)^2}\right) \nonumber
\end{align}
In this extrapolation model, the sensitivity parameters $\gamma_t$ affect both the mixture weights and the component means. The mixture weights for component $k$ increases as $\gamma_t$ approaches $\frac{\mu_{tk}(X)}{\sigma_{tk}}$.  
\end{example}

In general, we can apply the extrapolation factorization with logistic selection to observed data densities modeled with non-parametric Bayesian methods like Dirichlet process mixtures (DPM) of any exponential family distribution, and can can easily adapt the mixture results to model structured semi-continuous data as well.  In Section \ref{sec:analysis_jtpa}, we demonstrate both of these features by modeling zero-inflated income data, and use a DPM model for the continuous component.  

\subsection{Parameter Interpretations} 

%\avi{need to edit this section for clarity} The logistic-EF models include two sensitivity parameters:
Here, we discuss interpretations of the sensitivity parameters $(\gamma_0, \gamma_1)$ in the context where $s(Y(t)) = Y(t)$; that is, the sufficient statistic for the logistic selection model is simply $Y(t)$ itself.
In this setting, $\gamma_0$ and $\gamma_1$ are scalars, so we focus on interpreting their signs.
Put simply, $\gamma_0$ and $\gamma_1$ specify how potential outcome values are over- or under-represented among observed control and treated units. 
For example, $\gamma_1 > 0$ implies that units with large $Y(1)$ are over-represented among treated units, and the observed treated unit average is too large.
Likewise, $\gamma_0 > 0$ implies that units with large values of $Y(0)$ are more likely to be assigned to treatment, so the observed control unit average is too small.
A simple mnemonic for interpreting the sign of these parameters when $Y(t)$ is the sufficient statistic is that $\gamma_t$ has the same sign as the bias of the na\"ive estimate of the average treatment effect under that setting of the sensitivity parameters.
For any given setting of the sensitivity parameters, \eqref{eqn:mis data extrapolation} extrapolates from the observed to missing data by adjusting for the sampling bias implied by $\gamma_0$ and $\gamma_1$.
%This interpretation reveals the extrapolation factorization's roots in survey sampling and missing data, but may not be natural for causal inference.
%In causal inference, it is often more intuitive to reason about confounding from a complete-data perspective, so in this section, we consider scenarios under which a latent confounder could induce the types of selection bias encoded by different values of $(\gamma_0, \gamma_1)$. 

When interpreting the results of a sensitivity analysis, it is often useful to understand what sort of generating process could give rise to certain settings of the sensitivity parameters $(\gamma_0, \gamma_1)$.
We give several examples of such generating processes below.

\begin{example}[Same Sign]
Consider a study of a medical treatment with health outcome $Y$ and unmeasured income variable $U$.
%This implies positively correlated potential outcomes conditional on $X$.
Suppose that larger values of $Y$ correspond to good outcomes, higher income induces better outcomes (for example, $Y(t) = \alpha + \tau t + \psi U + \epsilon$ with $\psi > 0$) and that treatment is expensive, so $P(T = 1 \mid U)$ is increasing in $U$.
In this study, both $Y(0)$ and $Y(1)$ are positively correlated with $T$, so large values of $Y(1)$ are over-represented among the observed treated units, and large values of $Y(0)$ are under-represented among control units, corresponding to positive $\gamma_1$ and $\gamma_0$.  
When $\gamma_0$ and $\gamma_1$ have the same sign, the treatment and control group means are biased on opposite directions, so the ATE shows strong sensitivity when parameters are moved in this direction.
%then both $Y(0)$ and $Y(1)$ have positive correlation with $T$ of the same magnitude, and thus naturally in a logistic specification we would naturally propose $\gamma \triangleq\gamma_0 = \gamma_1$.
%One consequence of this is that, the ATC is increasing in $\gamma$ and the ATT is decreasing in $\gamma$.  As is evident in the example in Section \ref{sec:analysis_nhanes}, these two effects partially cancel out when estimating the ATE, and thus induce the \emph{appearance} of robustness of the ATE (despite sensitivity to confounders within each subgroup). 
\end{example}

\begin{example}[Opposite Signs]
Consider the canonical ```perfect doctor'' example \citep{rubin2003basic}, where a particular medical treatment is prescribed by a doctor who is able to perfectly predict $Y(0)$ and $Y(1)$ for each patient, and assigns the patient to whichever arm gives them the higher outcome.
Suppose that in this population $Y(1) - Y(0)$ is independent of $[Y(1) + Y(0)] / 2$; that is, the individual treatment effect for each student is unrelated to each individual's expected outcome under random assignment to treatment.
For example, suppose that $[Y(0), Y(1)]$ are independently normal.
Then the control arm and the treated arm both over-represent high outcomes, so $\gamma_0 < 0$ and $\gamma_1 > 0$. 
When $\gamma_0$ and $\gamma_1$ have opposite signs, the treated and control group means are biased in the same direction,so  the ATE shows relatively little sensitivity when the parameters are moved in these directions.
\end{example}

\begin{example}[Single-Arm Confounding]
Consider a study evaluating a job training program with wage outcome $Y$ where, prior to the study, a subset of units is randomly selected, and given access to an alternative program that they can attend if they do not enroll in the treatment, indicated by $U = 1$.
Suppose that
%(1) access to this alternative program is as-if-random after conditioning on covariates $X$,
the alternative program is beneficial on average (for example, suppose the potential outcomes are given by $Y(0) = \alpha(X) + \psi U + \epsilon$ with $\psi > 0$ and $Y(1) = \alpha(X) + \tau + \epsilon$), and units with access to the alternative program are less likely to enroll in treatment, so $P(T = 1 \mid U)$ is decreasing in $U$. 
Then, the observed outcomes under treatment would be representative of the distribution of $Y(1)$, so $\gamma_1 = 0$, but because of (1) and (2), units with higher wage outcomes would be over-represented under control, so $\gamma_0 < 0$.
\end{example}


%The logistic marginal selection functions we have introduced here have two sets of sensitivity parameters: $\gamma_0$ and $\gamma_1$.
%$\gamma_0$ is a sensitivity parameter affecting only the treatment effects of those assigned to control and $\gamma_1$ is a sensitivity parameter affecting only the treatment effects of the treated.  Unlike latent confounder formulations, our approach explicitly separates the sensitivity parameters for these two effects.  This makes it possible to encode a wide range of assumptions about the the effects of unconfoundedness.  To build intuition about the interpretations of these sensitivity parameters,
%We consider three cases: (1)  a case in which $\gamma \triangleq \gamma_0 = \gamma_1$, (2) a case in which $\gamma_1 = 0$ but $\gamma_0 \neq 0$ and (3) a case in which both sensitivity parameters are non-zero with  $\text{sign}(\gamma_0) = -\text{sign}(\gamma_1)$.
%We demonstrate interpretation by starting from a few simple complete data latent confounder models and deriving their implications in the extrapolation framework.  

%One simple example where case (1) arises is for models with a constant additive treatment effect, $\tau$, and complete data potential outcomes $Y(t) \mid X, U = \alpha(X) + \psi U + \tau t + \epsilon$.
%This implies positively correlated potential outcomes conditional on $X$.
%When the odds of treatment are increasing as function of $U$, then both $Y(0)$ and $Y(1)$ have positive correlation with $T$ of the same magnitude, and thus naturally in a logistic specification we would naturally propose $\gamma \triangleq\gamma_0 = \gamma_1$.  One consequence of this is that, the ATC is increasing in $\gamma$ and the ATT is decreasing in $\gamma$.  As is evident in the example in Section \ref{sec:analysis_nhanes}, these two effects partially cancel out when estimating the ATE, and thus induce the \emph{appearance} of robustness of the ATE (despite sensitivity to confounders within each subgroup). 

%For case (2), assume that $Y(0) \mid T, X, U = \alpha(X) + \psi U + \epsilon$ but that $Y(1)$ is conditionally independent of the latent confounder: $Y(1) \mid T, X, U = \alpha(X) + \tau + \epsilon$, where again $\tau$ represents the constant treatment effect.  This implies that the potential outcomes are independent, given $X$ and $\tau$. If we assume that the odds of treatment decrease with $U$, then $Y(0)$ is negatively correlated with $T$ (an hence we posit that $\gamma_0 < 0$), but $Y(1)$ is independent of $T$ (an hence $\gamma_1 = 0$).  In this setting, only the ATC is impacted by non-ignorable treatment assignment. Such a situation may arise if, for example, $U$ reflects the effect on the control potential outcomes from unobserved access to alternative treatments. It is plausible that access to better alternative treatments (as reflected by a large value of $U$), naturally reduces the propensity for assignment to treatment $T$.

%Finally, in case (3), we consider settings in which it might plausible for both sensitivity parameters are non-zero but of opposite sign.  In this setting, the potential outcomes are anti-correlated (conditional on $X$).  When $\gamma_0 > 0$ and $\gamma_1 < 0$ both the treatment effect among the treated and the treatment effect of the control are larger than they are under unconfoundedness.  Similarly, when $\gamma_1 < 0$ and $\gamma_1 > 0$ the treatment effect of the controls and the treatment effect of the treated are both smaller.  As we demonstrate in Section \ref{sec:analysis}, this leads to the largest changes in the ATE and QTEs.  Both cases (2) and (3) are consistent with what we refer to as ``selection on gains''. Under selection on gains, treatment assignment increase with unit level treatment effects.  A canonical illustration of this effect is described in the ``perfect doctor'' example, in which an oracular doctor prescribes the treatment only if it is beneficial \citep{rubin2003basic}. Under selection on gains, the magnitude of the estimated average treatment effect is exaggerated under the unconfoundedness assumption  (see Figure \ref{fig:1}). Estimated average and quantile treatment effect will weaken and possibly change sign, after correcting for selection on gains.

%In fact, as we show in Section \ref{sec:analysis}, treatment effects are most sensitive to selection effects when the sensitivity parameters are of opposite sign. 
%In, the complexity of MCMC inference limits analysis to binary confounder $U$. Because we separate the observed and unidentified components of the model, inference is much simpler and we allow much richer implicit model specifications for the distributions of a latent confounder $U$.  Although in this analysis we focused on the normal model, it is trivial to model $U$ as a different exponential family distribution, or even mixtures of exponential families, as shown in \citep{franks2016non}.  
%Such mixture exponential families include the normal-normal mixture, or the negative binomial (poisson response, gamma latent confounder). 

%Further, since U has zero variance given T, then $Cov(Y(0), Y(1)\mid T) = 0$.  

%By Equation \label{miss_dist_ef} we have

%\begin{align}
%f(Y(0) \mid T=1, X) &\propto f_{\text{normal}}(\alpha_0(X), %\sigma_0^2)*exp(\frac{\beta_0}{\sigma_0^2}Y(0))\\
%&= f_{\text{normal}}(\alpha_0(X) + \beta_0, \sigma_0^2)\\
%f(Y(1) \mid T=0, X) &\propto f_{\text{normal}}(\alpha_1(X) + \beta_1, %\sigma_1^2)*exp(\frac{-\beta_1}{\sigma_0^2}Y(0))\\
%&= f_{\text{normal}}(\alpha_1(X), \sigma_1^2)
%\end{align}


%Thus the ATT = $(\alpha_1(X) - \alpha_0(X)) + (\beta_1 -\beta_0)$ and the ATC = $ (\alpha_1(X) - \alpha_0(X))$ and Var(ATT) = Var(ATC) = $\sigma_0^2 + \sigma_1^2$

%Now assume that $\epsilon_{U_0} \sim [0, \sigma_{U_0}^2]$ and $\epsilon_{U_1} \sim [\phi,\sigma_{U_1}^2]$ are random variables.  If $\sigma^2_{U_0} = \sigma^2_{U_1}$ then the equations above hold and now the covariance between potential outcomes is positive (see equation ....).  

%Note that if $\sigma^2_{U_0} = \sigma^2_{U_1}$ are different, then the missingness mechanism is quadratic in the log odds (e.g. non-monotone):




% \avi{Can we put in a sub-section returning to estimands? It's sorta crazy that we just crank out a bunch of posterior draws of the potential outcomes and then calculate whatever estimands we want. This is certainly non-standard in other sensitivity approaches, so it seems worth highlighting that the workflow is to (1) create a machine for generating potential outcomes for a specified sensitivity parameter, then (2) estimate whatever contrast of those you want (within reason). Certainly a nice feature of this is that you can do one sensitivity analysis/Bayesian model for a whole bunch of different estimands at the same time}



% \avi{Are we going to comment on subgroups/heterogeneous treatment effects? Maybe I missed that somewhere?}



%These relationships elucidate the fact that logistic-EF models are \emph{conditional} models, as opposed to the latent confounder approaches discussed in Section \ref{sec:latent-confounder}, which are complete data models.  %Specifically, in the logistic-EF formulation, the observed and missing data distributions are each exponential family distributions (or mixtures thereof) in the same family, whereas in the latent confounder formulations we commonly assume the complete data is an exponential family distribution.  
%Specifically, if we start with the assumption that the two conditional distributions, $f(Y(t) \mid T)$ are exponential family distributions of the same form, this implies the treatment assignment mechanism is logistic in the sufficient statistics for that family.  By contrast, it is commonly assumed in the latent confounder models that the complete data potential outcomes and the marginal distribution of the latent confounder is of exponential family form (see Examples in Section \ref{sec:latent-confounder}). Often, this implies observed data distributions that are less tractable (e.g. the skew normal) and/or are are mis-specified due to partial identification. Below we provide several practical and simple example specifications and implications in the logistic-EF class.






\subsection{Calibrating Sensitivity Parameters}
\label{sec:calibration}

Well calibrated sensitivity parameters are essential to any sensitivity analysis.  
% As discussed extensively, 
In the extrapolation factorization, sensitivity parameters are completely unidentified, and thus we must reason about plausible values using prior knowledge and domain expertise. In order to facilitate this process for the logistic-EF model, we propose a method for calibrating the magnitudes of the sensitivity parameters.   Broadly, to calibrate sensitivity parameters we first estimate regression coefficients for observed covariates and then use these coefficients to anchor the sensitivity parameters, which also have regression coeficient interpretations. This approach is consistent with the calibration approaches used in latent confounder models \citep{imbens2003sensitivity, dorie2016flexible, blackwell2014selection, middleton2016bias, cinelli2018making}, with the important difference that our parameterization involves coefficients for the potential outcomes rather than for a latent confounder.  %Below we describe the details of the sensitivity calibration for the two model classes proposed in this section. 

%\hfill \break
%\textbf{Calibration in the Logistic-EF model:} 

% In the previous section we provided some high level interpretations of $\gamma_0$ and $\gamma_1$, based on their signs.  In addition to the broad interpretations, a meaningful analysis also require that the magnitudes of the parameters are well calibrated.  Our approach to calibration involves contextualizing the magnitude of the sensitivity parameters against the coefficients for observed covariates.  
In our setting, we consider a logistic regression of treatment on both of observed covariates and residual potential outcomes.  Let $R(t) =  (Y(t) - \alpha_t(X))$ be the potential outcomes after removing the effect of observed covariates.  %Intuitively, we presume some proportion of the variance in $R(t)$ is due to latent confounders that may effect the treatment assignment.  
%In other words, we treat $R(t)$ is a proxy for a latent confounder that is orthogonal to the observed $X$. 
In order to calibrate the coefficients we scale all predictors in the logistic regression to have unit variance so that they can be equitably compared.  We denote the unit scaled covariates as $\tilde{X}$ and the unit-scaled residuals $\tilde R(t) = \frac{R(t)}{\sigma_{rt}}$, where $\sigma_{rt}$ is the residual standard deviation.  We then posit that the unidentified treatment assignment mechanism can be expressed as
%
\begin{equation}
\label{eqn:logitef-calibration}
 f(T \mid Y(t), X) \sim \text{Bern}(\text{Logit}^{-1}( \beta \tilde X + \tilde{\gamma}_t\tilde R(t))) 
\end{equation}
%
where $\tilde \gamma_t$ corresponds to a change in log odds of being treated given a unit change in the rescaled residuals:
\begin{equation}
\label{eqn:tilde_gamma}
\tilde \gamma_t = \log \left(\frac{ \mathrm{odds}(T = 1 \mid \beta\tilde X, \tilde R(t) = r) }
{\mathrm{odds}(T = 1 \mid \beta\tilde X, \tilde R(t) = r - 1)}\right) \quad \forall r .
\end{equation}

\noindent Importantly, since $\tilde R(t)$ is orthogonal to $\tilde X$, estimates of $\beta$ are not affected by the inclusion of $\tilde R(t)$.  Thus, we can estimate the coefficients of the propensity score, $E[T\mid \tilde X] = \text{logit}^{-1}(\beta \tilde X)$, where  we let $\hat e(\tilde X)$ denote the fitted values of the logistic regression and $\hat \beta$ denote the estimated coefficients of that regression.  %Interestingly, for Bayesian inference of average treatment effects, estimates of the propensity coefficients $\beta$ are not strictly necessary although there is a large body of literature on improving efficiency through propensity score matching or reweighted methodology.  \avi{citations?}  
We use estimates of the propensity score coefficients as a baseline for calibrating a plausible range of values for $\tilde \gamma$.  For instance, if we posit that $\tilde \gamma_t = \hat \beta_j$ where $\hat \beta_j$ is the coefficients for the $j$th scaled feature, $\tilde X_j$, we assume that the effect of $\tilde R(t)$ on the log odds of $T$ is equal in magnitude and sign to the effect from $\tilde X_j$.  We can equivalently view $\exp(\tilde \gamma)$ as the odds ratio of treatment for two matched units that differ in $\tilde R(t)$ by 1.  

Ultimately, however, the logistic-EF approach parameterizes sensitivity in terms of a coefficient for the potential outcome $Y(t)$.  As such, we rewrite Equation \ref{eqn:logitef-calibration} as $f(T \mid Y(t), X) \sim \text{Bern}(\text{Logit}^{-1}(\hat \beta \tilde X - \frac{\tilde{\gamma}_t}{\sigma_{rt}}\tilde \alpha_t(X) + \frac{\tilde{\gamma}_t}{\sigma_{rt}} Y(t)))$.  We then use the value for $\gamma_t = \frac{\tilde{\gamma}_t}{\sigma_{rt}}$ to infer the missing data density (Equation \ref{miss_dist_ef}) and subsequently any causal estimands of interest.  In the additive logistic model, estimates of $\hat \beta \tilde X - \frac{\tilde{\gamma}_t}{\sigma_{rt}}\hat \alpha_t(X)$ have no impact on the inferred missing data density or causal estimates.
%
%\avi{Can we add back in some of the discussion from Jamie Robins (in his 2002 commentary on the Rosenbaum paper) talking about how $Y(0)$ is the ``ultimate confounder,'' so there's good precedent for parameterizing sensitivity this way}
%\noindent 
%Intuitively, $\tilde{\gamma}_t$ corresponds to the effect of $Y(t)$ on $T$ \emph{after} removing the effect due to observed covariates.
%

It should be noted that the described procedure is slightly complicated by the fact that the complete distribution of $R(t)$, the potential outcome residuals, is not estimable from the observed data and thus $\sigma_{rt}$ is also not directly estimable without assumptions.  In many model specifications, we assume the residual standard deviation in both the observed and missing data densities are identical, in which case $\sigma_{rt}$ is estimable (e.g. Equation \ref{eqn:norm_example_mis} for $\psi_t = 0$), but in more complex models, the residual standard deviation depends on the sensitivity parameters.  To make this explicit, we write $\sigma_{rt} =: \sigma_{rt}(\gamma_t)$.  In the logistic-EF models considered here, $\sigma_{rt}(\gamma_t)$ is usually available in analytic form.  Thus, for a calibrated value $\tilde{\gamma_t}$, we can solve for $\gamma_t$ as the solution to the equation $\tilde{\gamma}_t = \gamma_t\sigma_{yt}(\gamma_t)$ and use $\gamma_t$ to complete the specification for the missing data density $f^{\rm mis}(Y(t) \mid T=(1\-t), \gamma_t, X)$.  Residual standard deviations may differ for the treated and control potential outcomes, and when this is the case, calibration can be done separately for $\gamma_0$ and $\gamma_1$.  


%In practice, unless the selection effects are extreme, it is often sufficient to approximate $\sigma_{yt}$ with the observed data standard deviation when calibrating.  
% In Algorithm \ref{algo:ef-calibration} we summarize the procedure for calibrating and estimating effects, and in Section \ref{sec:analysis_nhanes} we provide a concrete applied example of calibration in the logit-EF model.

% %Since the purpose of rescaling is to facilitate interpretation precise estimates of $\sigma_{yt}(\gamma_t)$ are not essential and   

% %In this analysis, the complete data distribution of $Y(t)$ is a two component mixture of the observed density \ref{eqn} and missing data density \ref{eqn}, and thus we can easily derive $\sigma_{yt}(\gamma_t)$ using the law of total variance.
% \begin{algorithm}
% \caption{Sensitivity Parameter Calibration in the Logistic-EF Model}
%   \begin{enumerate}
%     \item Fit a logistic regression on the unit-scaled covariates, $\tilde X$, to estimate the coefficients $\hat{\beta}$
%     \item Calibrate $\tilde{\gamma_t}$ relative to the coefficients $\hat{\beta}$ (using the interpretation given in \ref{eqn:tilde_gamma})
%     \item Find $\gamma_t$ as the solution to $\tilde{\gamma}_t = \gamma_t\sigma_{yt}(\gamma_t)$
%     \item Compute $f(Y(t) \mid T = (1 - t),  \gamma_t, X)$, estimate treatment effects.
% \end{enumerate}
% \label{algo:ef-calibration}
% \end{algorithm}

%Note that in practice, when $\gamma_t$ is relatively small, $\frac{Var(Y(t))}{Var(Y(t) \mid T=t)} \approx 1$ and thus, we can simplify things by calibrating $\gamma_t$ using only the variance of the \emph{observed} distribution of $Y(t)$. 




==> sections/sec-latent-confounder.tex <==
\section{Difficulties with Complete-Data Models}
\label{sec:latent-confounder}

%The primary motivation for the sensitivity analysis approach explored in this paper is to enforce a clean separation between identified and unidentified portions of the working model.
%In this section, we discuss why this separation is important, and show that this separation is difficult to achieve in general using complete-data models.
In this section, we discuss some difficulties with \emph{latent confounder models}, a popular complete-data modeling approach to sensitivity analysis that explicitly models unobserved confounders as latent variables.
\revs{Despite their popularity, this setup remain poorly understood; to quote \citet[][Chapter 7]{gustafson2015bayesian} in his discussion of these models, ``The crux of the situation is that we lack theoretical insight into even quite basic questions about what is going on.''}
We provide some theoretical insight here, showing that, in general, it is difficult to specify latent confounder models so that the sensitivity parameters are uninformed by the observed data.
This difficulty motivates our distinct approach to sensitivity analysis, which we discuss in the next section.
% Readers primarily interested in the details of our approach can skip this section.

%As we discuss, sensitivity parameters that are fully or partially identified complicate both the interpretation and practical application of sensitivity analysis.

\subsection{Latent Confounder Models} % and Implied Observed Outcome Distribution}
Latent confounder modeling is a common approach for sensitivity analysis in causal inference and have a long history \citep{rosenbaum1983assessing}.
% proposed the modern form of the latent confounder model to sharpen bounds derived in the pioneering work of \citet{cornfield1959smoking} in the debate over the causal effect of smoking and lung cancer.
%
Generally, latent confounder models assert that unconfoundedness would hold if only an additional latent confounder $U$ were observed; that is, for some latent variable $U$, $(Y(0), Y(1)) \independent T \mid U, X$.
The model then simultaneously specifies the conditional distributions of treatment and potential outcomes given $X$ and $U$.
This marks a departure from selection and pattern-mixture factorizations, which model treatment and potential outcomes sequentially.
In latent variable models, dependence on the latent variable $U$ is indexed by a vector of sensitivity parameters $\psi = (\psi_{Y_0}, \psi_{Y_1}, \psi_T)$.
%This formulation implies a complete-data model $f_\psi([Y(0), Y(1)], T \mid X)$ when the latent confounder is integrated out.
%Usually, we also assume that $U \independent X$.
The full model specification is
%
\begin{align*}
U \mid X &\sim f(U \mid X)\\
T \mid U, X &\sim f_{\psi_T}(T \mid X, U)\\
f_{\psi_T}(T \mid X, U) &= \text{Bern}(e_{\psi_T}(X, U))\\
Y(t) \mid U, X &\sim f_{\psi_{Y_t}}(Y(t) \mid X, U) 
\end{align*}
\noindent where $f(U \mid X)$ is the density of the latent confounder; $f_{\psi_{Y_t}}(Y(t) \mid X, U)$ is the potential outcome distribution for treatment $t$ given the observed and latent variables; and  $e_{\psi_T}(X, U)$ is the probability of receiving treatment given both $X$ and $U$, written with $e(\cdot)$ invoke a parallel to the propensity score.
Here, the sensitivity parameters $\psi$ encode how the treatment and potential outcomes depend on the unobserved confounder.  A common assumption is that $\psi_Y = \psi_{Y_0} = \psi_{Y_1}$, which means that the effect of the latent confounder on the potential outcome is the same in each treatment arm.  For sensitivity analysis, latent confounder models are usually parameterized so that some specific values of the sensitivity parameters $\psi$ indicate the ``no unobserved confounding'' case.
This occurs whenever $f_{\psi_T}(T \mid X, U)$ does not depend on $U$ or when $f_{\psi_{Y_t}}(Y(t) \mid X, U)$ is free of $U$ for both $t \in \{0,1\}$.  
%Often the parameter value $\psi_\cdot = 0$ is used to represent no dependence on $U$.

Despite their intuitive appeal, latent confounder models often imply observed outcome distributions that depend on sensitivity parameters in ways that are not fully transparent. 
%For this reason, it is difficult in general to specify latent confounder models with unidentified sensitivity parameters.
The observed outcome distribution in each arm $t \in \{0,1\}$ has the following form:
\begin{align}
%f(T \mid X) &= \int_{\mathcal U} f_{\psi_T}(T \mid X, U) f(U) dU\\
f^{\rm obs}_{\psi,t}(Y(t) \mid X, T=t) &= \int_{\mathcal U} f_{\psi_{Y_t}}(Y(t) \mid X, U) f_{\psi_T}(U \mid X, T=t) dU \label{eqn:obs PO distribution}.
\end{align}
The distribution of observed outcomes is a mixture over the mixing measure $f_{\psi_T}(U \mid X, T = t)$. 
%Because of this complicated form, it is difficult to reason about how the observed outcome distribution depends on $\psi_T$ and $\psi_{Yt}$. 
Depending on the specification, the sensitivity parameters $\psi$ are often partially, if not fully, identified. 
%For this reason, specifying an invariant parameterization, such that $f^{\rm obs}_\psi(Y(t) \mid X, T=t) = f^{\rm obs}(Y(t) \mid X, T=t)$ is very difficult in the latent confounder models.  




%In this section, we give conditions under which the observed-data distribution $f(Y^{obs}, T)$ identifies the sensitivity parameters in latent conoufnder formulations.  
%We show identification by decomposing the observed data density into the two following factors.


%\noindent The mixing measure in \eqref{eqn:PO_distribution} is the conditional distribution of $U$ given $T$ and $X$, given by
%
%\begin{equation}
%\label{eqn:confounder_conditional}
%f_{\psi_T}(U \mid X, T) = \frac{f_{\psi_T}(T\mid U, X)f(U \mid X)}{\sum_{t\in\{0,1\}} f_{\psi_T}(t\mid U, X)f(U \mid X)}.
%\end{equation}
%
%Under this decomposition, confounding is induced by the two factors of the integrand in \eqref{eqn:PO_distribution}, which are parameterized by sensitivity parameters $\psi_T$ and $\psi_{Yt}$.
%Confounding is present, in the sense that the observed outcomes are not representative of missing outcomes
%$$
%f(Y(t) \mid X, T=t) \neq f(Y(t) \mid X, T = 1-t)
%$$
%when the following two conditions hold:
%\begin{enumerate}
%\item For at least one $t \in \{0,1\}$, the conditional outcome distribution depends on $U$, so that
%$$f_{\psi_{Y_t}}(Y(t) \mid X, U = u, T) \neq f(Y(t) \mid X, T)$$
%\item The mixing measure differs depending on the value treatment indicator, so that $$f_{\psi_T}(U\mid X, T = t) \neq f(U \mid X).$$
%\end{enumerate}
%The first condition requires that the potential outcome distributions have different mixture components for different values of $U$.
%The second condition states that the distribution of the latent confounder differs between the groups assigned treatment and control.
%Note that this second condition is equivalent to stating that $f_{\psi_T}(T \mid X, U)$ does not depend on $U$. 

\subsection{A Simple Example of Sensitivity Parameter Identification}

Before we turn to a general treatment of sensitivity parameter identification in latent confounder models, we give a simple example of a case where identification occurs, and the complications that arise as a result.

\begin{example}[Normal Outcome, Binary Confounder]
\label{ex:normal outcome binary confounder}
Suppose we have a study with a continuous outcome and no covariates.
We make the assumption that treatment was randomly assigned according to a Bernoulli design, but it is plausible that there exists a latent class that confounds the study.  To test the robustness of our conclusions to the presence of such a latent class, we propose a sensitivity analysis by introducing a binary latent confounder.  The model is parameterized as follows: 
\begin{align*}
U &\sim \Bern(\xi_u)\\
T \mid U &\sim \text{Bern}(g(\alpha + \psi_T U))\\
Y(t) \mid U &\sim N(\mu_{t} + \psi_Y U, \sigma^2).
\end{align*}
When $(\psi_T, \psi_{Y}) = (0, 0)$, the model reduces to random assignment to treatment. The observed data distribution depends on the sensitivity parameters $\psi$.
To see this, let $h_{\psi_T} := P(U = 1 \mid T)$.
By Equation \ref{eqn:obs PO distribution}, the distribution of observed outcomes is a two-component mixture of normals for $t = \{0,1\}$:
%to note the dependence on relevant parameters and observables.  %We can integrate out the binary $U$ 
\begin{align}
\label{eqn:dorie_model}
%U \mid T &= Bern\left(\left[\frac{\pi_U \Phi(\beta X + \phi)}{\pi_U \Phi(\beta X + \phi) + (1-\pi_U) \Phi(\beta X)}\right]^T\right)\\
%U\mid X, T &= Bern(\pi_{uT}(X))\\
Y(t) \mid T=t &\sim h_{\psi_T}N(\mu_{t} + \psi_Y, \sigma^2) + (1-h_{\psi_T})N(\mu_{t}, \sigma^2)
\end{align}
%
\noindent The observed and missing potential outcome distributions, $f(Y(t) \mid T = t, X)$ and $f(Y(t) \mid T = 1-t, X)$, respectively, have the same mixture components but different mixture weights.
$\psi_Y$ determines the difference between the component means.
%Here, $\pi_u$ depends on $\psi_Y$ and one of the mixture component means depends on $\phi$.
The mixture weights, $h_{\psi_T(t)}$ and component means are identifiable under relatively weak assumptions \citep[see][]{everitt1985mixture}.

In Figure~\ref{fig:misfit}, we demonstrate a range of data fits obtained from this model.\footnote{In this simulation we set $\xi_u = 1/2, \alpha=0, \mu_t=0, \psi_T=-1, \psi_Y=5$ and $\sigma^2=1$.}
As is common practice, we fit the model multiple times for a range of sensitivity parameters.
In Figure \ref{y0mis} we plot the true (blue) and inferred (red) observed potential outcome densities for the control potential outcomes. 
Most settings of the sensitivity parameters result in severe misfit of the observed data, and would likely be rejected by a competent analyst if they were considered the ``main'' model for the observed data.
In this case, the sensitivity analysis operates as a model checking exercise more than as an exploration of relaxed identification assumptions. 
In fact, based on this parametric specification, the investigator could reject the hypothesis that the study satisfies Assumption~\ref{assn:unconfounded} based on model fit, but could still estimate the causal effect because all parameters of the mixture model are identified.

\end{example}

\begin{figure}	
	\centering
	\begin{subfigure}[t]{0.47\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figs/Y0_misspec.pdf}
		\caption{$Y(0) \mid T=0$}\label{y0mis}		
	\end{subfigure}
	\quad\quad
	%\begin{subfigure}[t]{2.5in}
	%	\centering
	%	\includegraphics[width=2.0in]{figs/Y1_misspec.pdf}
	%	\caption{$Y(1) \mid T=1$}\label{y1mis}
	%\end{subfigure}
	\begin{subfigure}[t]{0.47\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{figs/pp_bin_norm_plot_1.pdf}
	    \caption{$\mu_{Y^{obs}}(X, 0)$  \label{fig:binary outcome normal confounder}}
    \end{subfigure}
	\caption{Illustrations of sensitivity parameter identification in two sensitivity models (Example 1 and Example 2), via variation in posterior predictive distributions at different sensitivity parameter settings.
	(a) True (blue) and inferred (red) observed control outcome densities, $f(Y(0) \mid T=0)$, implied by the normal outcome-binary latent confounder model with sensitivity parameters $\psi_T$ and $\psi_Y$ (Example 1). $\Delta \psi_T$ and $\Delta \psi_y$ represent the difference between the true and assumed sensitivity parameters.  The observed data densities are only correctly inferred when we assume the true values of the sensitivity parameters $(i.e. \Delta \psi_T = \Delta \psi_Y = 0$). Note that the true potential outcome distributions $Y(0)$ are a mixture of normals with the same component means and different variances.
	(b) Posterior predictive expectation functions for observed control outcomes in the binary outcome-normal confounder model with a covariate $X$ (Example 2).
	Solid line shows posterior expectation; shading shows a pointwise 50\% posterior predictive interval.
	When either sensitivity parameter $\psi_T$ or $\psi_{Y0}$ is equal to zero, the surface is monotonic, but when their signs differ, the surface shows non-monotonicity.
	\label{fig:misfit}}
\end{figure}


More elaborate forms of the model in Example~\ref{ex:normal outcome binary confounder} appear throughout the literature, including extensions that incorporate covariates.
\citet{imbens2003sensitivity} first proposed a linear model for the mean of the potential outcomes, $\mu_{Xt} = \tau t + \gamma X$; \citet{dorie2016flexible} extended Imbens' approach and instead model $\mu_{Xt}$ using Bayesian Adapative Regression Trees.
Under these specifications, the residuals of the observed outcomes $Y(t) - E[Y(t) \mid X, T = t]$ are distributed as a mixture of normals, and the identification issue noted in Example~\ref{ex:normal outcome binary confounder} remains.

%We will return to Example~\ref{ex:normal outcome binary confounder} below.
%Given that all parameters in this model are identified, one could just as easily specify this latent confounder model as the ``main'' working model, and perform a valid sensitivity analysis based on this model fit.
%In Section~\ref{sec:mix-model}, we specify a valid sensitivity analysis tailored to this finite Gaussian mixture specification.

\subsection{Sensitivity Parameter Identification in General}
To close this section, we discuss conditions under which sensitivity parameters in latent confounder models are at least partially identified.
The purpose of this discussion is to emphasize that, unless strong restrictions are put on on the sensitivity model, latent confounder models will generally define sensitivity parameters that are informed by the data.
In some cases, these restrictions may encourage investigators to use less-than-ideal models for their observed data so that they can perform a valid sensitivity analysis, or the restrictions may discourage investigators from performing sensitivity analysis at all.

We study the observed outcome model in \eqref{eqn:obs PO distribution} as a mixture model to show that identification occurs under rather weak conditions. 
Identification in mixture models is a well-studied problem.
\citet{Hennig2000} contains a thorough reference list, with general treatments of the problem given by \citet{teicher1960}, \citet{chandra1977}, and \citet{rao1992}.
\citet{everitt1985mixture} gives an accessible review of identification in the case of finite mixtures.

For our discussion in this section, we focus on partial identification, where the observed data distribution contains information that narrows down possible values for the sensitivity parameters.
We formalize this information in terms of incompatibility between the observed data distribution and the complete data distribution induced by certain settings of the sensitivity parameters.

\begin{definition}[Incompatibility]
We say the observed data distribution $f(Y^{\rm obs}, T \mid X)$ is \emph{incompatible} with a sensitivity parameter setting $\tilde \psi$ iff there exists no complete data model $f_{\tilde \psi}(Y(0), Y(1), T \mid X)$ with sensitivity parameters $\tilde \psi$ that implies $f(Y^{\rm obs}, T \mid X)$.
\end{definition}

We say that a sensitivity parameter is partially identified if the model family can induce observed data distributions that are incompatible with some values of the sensitivity parameters.
For example, in the context of Example~\ref{ex:normal outcome binary confounder}, the latent confounder model can induce multimodal observed outcome densities, but such densities are incompatible with the setting $\tilde \psi_Y = 0$. 
Thus, $\psi_Y$ is partially identified; one could, in principle, reject this sensitivity parameter value on the basis of a test of unimodality for the observed data densities.

%, and let $\mathcal D$ be the family of latent confounder distributions $f_{\psi_T}(U \mid T)$.

%\begin{condition}[Sufficient Condition for Partial Identification]
%\label{def:partial identification}
%The sensitivity parameters $\psi$ in a latent confounder model are partially identified if, for some $t \in \{0, 1\}$ there exists some observed outcome distribution $f_m \in \mathcal M_t$ and sensitivity parameter setting $\tilde \psi := (\tilde \psi_T, \tilde \psi_{Yt})$ such that $f_m$ is incompatible with $\tilde \psi$.
%
%there exists no combination of conditional outcome distributions $f_c \in \{f_{\psi_{Yt}} \in \mathcal C : \psi_{Yt} = \tilde \psi_{Yt}\}$ and mixing measures $f_d \in \{f_{\psi_T} \in \mathcal D : \psi_T = \tilde \psi_T\}$ that satisfy 
%\begin{align}
%f_m(Y^{obs} \mid T, X) = \int_{\mathcal U} f_c(Y^{obs} \mid T, U, X) f_d(U \mid T, X) dU\label{eqn:partial mixture condition}.
%\end{align}
%\end{condition}

Here, we show that partial identification occurs under fairly weak conditions on the latent confounder model.
Stronger results regarding point identification under more restrictive parametric assumptions are available in the references cited above.
Following \citet{chandra1977}, we state our conditions in terms of model families.
Let $\mathcal M_t$ be the family of observed data distributions $f^{\rm obs}_{\psi, t}(Y(t) \mid T=t, X)$ and let $\mathcal C_t$ be the family of conditional outcome distributions $f_{\psi_{Yt}}(Y(t) \mid U=u, X)$.
Recall that, by \eqref{eqn:obs PO distribution}, the members of $\mathcal M_t$ are mixtures over the members of $\mathcal C_t$.

\begin{proposition}[Sufficient Condition for Partial Identification of Sensitivity Parameters]
\label{prop:partial identification}
Suppose the following two conditions hold:
\begin{itemize}
\item $\mathcal M \supset \mathcal C$, so that the mixture outcome distribution has a strictly larger model family than the conditional outcome distribution, and
\item There exist sensitivity parameter settings $\tilde \psi$ such that $f_{\tilde \psi_{Yt}}(Y(t) \mid U, X)$ does not depend on $U$, or such that $f_{\tilde \psi_T}(U \mid T)$ is degenerate.
\end{itemize}
Then the sensitivity parameters $\psi$ are partially identified.
\begin{proof}
For any setting $\tilde \psi$ that satisfies the second condition, the corresponding mixture distribution $f^{obs}_{\tilde \psi, t}(Y(t) \mid T, X)$ must lie within $\mathcal C$.
Thus, any mixture distribution $f_m \in \mathcal M \setminus \mathcal C$ is incompatible with these sensitivity parameter settings, so the sensitivity parameter is partially identified.
\end{proof}
\end{proposition}

%We demonstrate visually how the sensitivity parameters change the observed data distribution in Figure~\ref{fig:binary outcome normal confounder}.
% 
% \begin{remark}
% \avi{Check this} 
Proposition~\ref{prop:partial identification} is important because it outlines cases in which the parametric specification of the sensitivity model makes it possible to reject unconfoundedness using the observed data.
% The case constructed in the proof of Proposition~\ref{prop:partial identification} is particularly important, because it indicates that under the conditions of the theorem, it is possible to reject unconfoundedness based on the observed data on the basis of the parametric specification of the sensitivity model.
% \end{remark}
%
The conditions in Proposition~\ref{prop:partial identification} are weak, but not universal.
The second condition is almost always satisfied by design because it corresponds to having settings of the sensitivity parameters that represent the unconfounded case.
The first condition, however, depends on the sample space of $Y^{\rm{obs}}$ and the parametric specification, and does not hold in some common specifications.
For example, in the sensitivity analysis of \citet{rosenbaum1983assessing}, the outcomes and latent confounder are binary and sensitivity parameters are not shared across covariate strata  \citep[see also][]{jung2018algorithmic}.
In this case, within each covariate stratum, mixtures of Bernoulli random variables are themselves Bernoulli so $\mathcal M = \mathcal C$, and the sensitivity parameters are unidentified.
However, in the common case where sensitivity parameters are shared across covariate strata, the condition holds, even when outcomes are binary.
We demonstrate this in the following example.

\begin{example}[Binary Outcome with Covariates]
Consider a latent confounder model with binary outcomes.
We posit the existence of a normally distributed latent confounder:
%
\begin{align}
U &\sim N(0, 1)\\
%\pi_t &= \Phi \left( \frac{\psi_T}{ \sqrt{1+\psi_T^2} } \right)\\
%f(U \mid T=1) &\propto \phi(U)\Phi(\psi_T + \psi_T U)\\
%\pi_{Y(t)_{\text{obs}}} &= E[g(\beta_t + \psi_Y U) \mid T = t]
T \mid U, X &\sim \Bern(g(\beta X + \psi_T U))\\
Y(t) \mid U, X &\sim \Bern(\mu_{Yt}(X, U))\label{eqn:normalU binary outcome}\\
\mu_{Yt}(X, U) &= g(\alpha X + \psi_Y U)
\end{align}

Here, the observed outcome distribution is Bernoulli, and characterized by the function
$$
\mu_{Y^{obs}}(X, t) = E[Y(t) \mid T = t, X] = \int_{\mathcal U} \mu_{Yt} f(U \mid T=t, X) dU.
$$

\noindent
%where $f_u(U \mid T)$ is known as the extended skew normal distribution \citep{azzalini2005skew}.
%Again, $\pi_t$ is a continuous monotonic function of $\psi_T$ for any fixed $\alpha$.
%$\alpha$ is not identified from the observed data, but for $\alpha$ fixed to any value, $\psi_T$ is identified.
%Similarly we can use equation \ref{eqn:obs_distribution} to argue that $\pi_{Y(t)_{\text{obs}}}$ is monotonic in $\beta_t$, $\psi_Y$ is completely unidentified and that $\beta_t$ is identified given $\psi_Y$.
In this example, $\mathcal C$ is a smaller family than $\mathcal M$.
In particular, the family $\mathcal C$ only contains distributions whose mean function $\mu_{Yt}$ is monotone in $X$, given the linear dependence in $\mu_{Yt}$ and the monotonicity of $g$.
Meanwhile, the family $\mathcal M$ contains distributions whose mean function $\mu_{Y^{obs}}(X, t)$ can be non-monotone in $X$ because of the indirect dependence on $X$ introduced by the mixing measure $f(U \mid T=t, X)$.
This non-monotonicity is particularly pronounced when $\psi_T$ and $\psi_{Yt}$ have opposite sign for at least one of $t \in \{0, 1\}$.
%
We demonstrate how the posterior predictive distribution of observed data varies as a function of the sensitivity parameters in this model in Figure~\ref{fig:misfit}.
\citet[][Chapter 7]{gustafson2015bayesian} discusses more general versions of this example, noting that there is no general strategy for separating information about parameters $(\alpha, \beta)$ and the sensitivity parameters $\psi$ in a transparent way.
\end{example}

\revs{Finally, several authors have proposed complete-data sensitivity models with unidentified sensitivity parameters, most of which require binary or categorical outcomes \citep{rosenbaum1983assessing,ROBINS_NON_1997,Vansteelandt_Ignorance_2006,Daniels_Missing_2008}.
However, as we have demonstrated in this section, this non-identification is difficult to achieve in general, may require non-trivial reparameterization, and is fragile when attempting to generalize these sensitivity analysis methods.
This motivates the sensitivity analysis framework we present below, whose guiding principle is clean separation of observable and unobservable model implications.} 
